IELM: An Open Information Extraction Benchmark for Pre-Trained Language Models

We introduce a new open information extraction (OIE) benchmark for pre-trained language models (LM). Recent studies have demonstrated that pre-trained LMs, such as BERT and GPT, may store linguistic and relational knowledge. In particular, LMs are able to answer ``fill-in-the-blank'' questions when given a pre-defined relation category. Instead of focusing on pre-defined relations, we create an OIE benchmark aiming to fully examine the open relational information present in the pre-trained LMs. We accomplish this by turning pre-trained LMs into zero-shot OIE systems. Surprisingly, pre-trained LMs are able to obtain competitive performance on both standard OIE datasets (CaRB and Re-OIE2016) and two new large-scale factual OIE datasets (TAC KBP-OIE and Wikidata-OIE) that we establish via distant supervision. For instance, the zero-shot pre-trained LMs outperform the F1 score of the state-of-the-art supervised OIE methods on our factual OIE datasets without needing to use any training sets. Our code and datasets are available at https://github.com/cgraywang/IELM

==> appendices_table/unmapped_bertlarge_kbp.tex <==
SF13\_ENG\_001 & Bashardost was born in 1965 in the southern Ghanzi province and his family migrated to Iran and then to Pakistan after successive coup and factional fighting in Afghanistan . & (Bashardost, in, The Southern Ghanzi Province) $\rightarrow$ (Ramazan Bashardost, per:stateorprovince\_of\_birth, The Southern Ghanzi Province)\\ \hline
SF13\_ENG\_012 & Gadahn , also known as Azzam the American , was born in 1978 . & (Gadahn, ,, Azzam) $\rightarrow$ (Adam Gadahn, per:alternate\_names, Azzam)\\ \hline
SF13\_ENG\_015 & Besides her sister , Philip , survivors include a son , Graham ; three daughters , Sidney , Gillian and Alexia ; and three grandchildren . & (Her Sister, ,, Philip) $\rightarrow$ (Lucille Clifton, per:siblings, Philip)\\ \hline
SF13\_ENG\_015 & The poet laureate of Maryland from 1979 to 1985 , Clifton was a writer in residence at Coppin State College , now Coppin State University , a historically black college in Baltimore . & (Clifton, in, Coppin State College) $\rightarrow$ (Lucille Clifton, per:school\_attended, Coppin State College)\\ \hline
SF13\_ENG\_015 & Her father , Samuel , was a steelworker ; her mother , Thelma , worked in a laundry . & (Her Father, ,, Samuel) $\rightarrow$ (Lucille Clifton, per:parents, Samuel)\\ \hline
SF13\_ENG\_015 & Lucille Clifton , a distinguished American poet whose work trained lenses wide and narrow on the experience of being black and female in the 20th century , exploring vast subjects like the indignities of history and intimate ones like the indignities of the body , died on Saturday in Baltimore . & (Lucille Clifton, ,, poet) $\rightarrow$ (Lucille Clifton, per:title, poet)\\ \hline
SF13\_ENG\_015 & The precise cause of death had not been determined , her sister , Elaine Philip , told The Associated Press on Sunday . & (Her Sister, ,, Elaine Philip) $\rightarrow$ (Lucille Clifton, per:siblings, Elaine Philip)\\ \hline
SF13\_ENG\_037 & CLAUDE CHABROL , PIONEER FRENCH FILMMAKER , DIES AT 80 Joseph Berger contributed reporting from New York , and Maia de la Baume contributed from Paris . & (Claude Chabrol, ,, Pioneer French Filmmaker) $\rightarrow$ (Claude Chabrol, per:title, Pioneer French Filmmaker)\\ \hline
SF13\_ENG\_037 & Chabrol ' s survivors also include his third wife , Aurore Pajot , who acted as his script supervisor on nearly all of his movies from 1968 on and whom he married in 1981 ; and Pajot ' s daughter , Cecile Maistre , who was an assistant director on his films and wrote the script with him for " The Girl Cut in Two " ( 2007 ) . & (His Third Wife, ,, Aurore Pajot) $\rightarrow$ (Claude Chabrol, per:spouse, Aurore Pajot)\\ \hline
SF13\_ENG\_044 & Dominick Dunne , a novelist and journalist who chronicled true - crime tales of the rich and infamous , including O . J . Simpson and Claus von Bulow , and in turn became a celebrity in his own right , died of bladder cancer Aug . 26 at his home in New York City . & (Dominick Dunne, ,, A Novelist) $\rightarrow$ (Dominick Dunne, per:title, A Novelist)\\ \hline
SF13\_ENG\_044 & Dunne and his wife , Ellen Griffin Dunne , known as Lenny , were married in 1954 . & (His Wife, ,, Ellen Griffin Dunne) $\rightarrow$ (Dominick Dunne, per:spouse, Ellen Griffin Dunne)\\ \hline
SF13\_ENG\_044 & Dunne was born in 1925 in Hartford , Connecticut , to a wealthy Roman Catholic family and grew up in some of the same social circles as the Kennedys . & (Dunne, ,, Connecticut) $\rightarrow$ (Dominick Dunne, per:stateorprovince\_of\_birth, Connecticut)\\ \hline
SF13\_ENG\_049 & A professor emeritus at Yale University , Mandelbrot was born in Poland but as a child moved with his family to France where he was educated . & (Mandelbrot, ,, Yale University) $\rightarrow$ (Benoit Mandelbrot, per:employee\_or\_member\_of, Yale University)\\ \hline
SF13\_ENG\_058 & Access Industries , a privately held company founded in 1986 by Len Blavatnik , has a diverse portfolio of investments in industry , real estate , media and telecommunications . & (Access Industries, ,, A Privately Held Company) $\rightarrow$ (Access Industries, properties, A Privately Held Company)\\ \hline
SF13\_ENG\_079 & Water and its links to development , peace and conflict were key words in the annual sessions , Anders Berntell , executive director of Stockholm International Water Institute ( SIWI ) , said in his opening address . & (Stockholm International, ,, Anders Berntell) $\rightarrow$ (Stockholm International Water Institute, per:top\_members\_or\_employees, Anders Berntell)\\ 

==> appendices_table/unmapped_bertlarge_wikidata.tex <==
Nick\_Aldis & He was also a co - presenter of " Britain ' s Strongest Man " on Challenge TV in the United Kingdom . & (Challenge Tv, in, The United Kingdom) $\rightarrow$ (Challenge TV, in, united\_kingdom.Q145)\\ \hline
Douglas\_Bader & At the age of two , Bader joined his parents in India for a year . & (His Parents, in, India) $\rightarrow$ (douglas\_bader.Q348780, in, india.Q668)\\ \hline
Douglas\_Bader & He remained in France after the war , where , having attained the rank of major , he died in 1922 of complications from those wounds in a hospital in Saint - Omer , the same area where Bader would bail out and be captured in 1941 . & (He, in, France) $\rightarrow$ (douglas\_bader.Q348780, in, france.Q142)\\ \hline
Douglas\_Bader & On 2 July 1941 he was awarded the bar to his DSO. & (He, was awarded the bar, his DSO) $\rightarrow$ (douglas\_bader.Q348780, was awarded the bar, distinguished\_service\_order.Q615838) \\ \hline
Helen\_Storrow & His father , also named James Jackson Storrow , was a prominent attorney , whose clients included Alexander Graham Bell and the government of Venezuela ; his mother , Ann Maria Perry , was the grandchild of naval hero Commodore Oliver Hazard Perry , and a distant cousin of President Thomas Jefferson . & (His Father, was, A Prominent Attorney) $\rightarrow$ (His Father, occupation.P106, lawyer.Q40348)\\ \hline
Helen\_Storrow & Helen Storrow Helen Osborne Storrow was a prominent American philanthropist , early Girl Scout leader , and chair of the World Committee of the World Association of Girl Guides and Girl Scouts for eight years . & (Helen Osborne Storrow, was, A Prominent American Philanthropist) $\rightarrow$ (helen\_storrow.Q5703224, place\_of\_birth.P19, united\_states.Q30)\\ \hline
Jacob\_Van\_Ruisdael & His cousin Jacob was a registered Mennonite in Amsterdam . & (His Cousin, was, A Registered Mennonite) $\rightarrow$ (His Cousin, was, A Registered Mennonite)\\ \hline
Jacob\_Van\_Ruisdael & He appears to have been strongly influenced by other contemporary local Haarlem landscapists , most notably Cornelis Vroom and Allaert van Everdingen . & (He, have been strongly influenced by, landscape painting) $\rightarrow$ (jacob\_van\_ruisdael.Q213612, have been strongly influenced by, landscape\_art.Q191163)\\ \hline
Liaquat\_Ali\_Khan & Liaquat Ali Khan was educated at the Aligarh Muslim University in India , and then at Oxford University in the United Kingdom . & (Liaquat Ali Khan, in, India) $\rightarrow$ (liaquat\_ali\_khan.Q295713, in, india.Q668)\\ \hline
Pauline\_Baynes & Baynes began her education at a convent school . & (Her Education, at, A Convent School) $\rightarrow$ (pauline\_baynes.Q101951, at, catholic\_school.Q1138671)\\ \hline
Pauline\_Baynes & Her most vivid recollection of their New Year ' s Eve lunch at Magdalen College was of his gleefully picking nuts out of a bowl of Brussels sprouts . & (Their New Year'S Eve Lunch, at, Magdalen College) $\rightarrow$ (pauline\_baynes.Q101951, at, magdalen\_college,\_oxford.Q81162)\\ \hline
Pauline\_Baynes & By the time that she left , she had already formed the ambition of becoming an illustrator . & (She, formed the ambition of becoming, An Illustrator) $\rightarrow$ (pauline\_baynes.Q101951, formed the ambition of becoming, illustrator.Q644687)\\ \hline
Thor\_Heyerdahl & He was an atheist . & (He, was, An Atheist) $\rightarrow$ (thor\_heyerdahl.Q133622, was, An Atheist)\\ \hline
Thor\_Heyerdahl & He is buried in the garden of the family home in Colla Micheri . & (He, is buried, Colla Micheri) $\rightarrow$ (thor\_heyerdahl.Q133622, is buried, colla\_micheri.Q3647771)\\ \hline
Neville\_Southall & He moved on to Cheshire County League club Winsford United at the age of 20 . & (He, to, Cheshire County League Club Winsford United) $\rightarrow$ (neville\_southall.Q436650, to, winsford\_united\_f.c..Q5213266)\\ \hline
Neville\_Southall & He later became a player - coach at York City , Rhyl , Shrewsbury Town and Dagenham \& Redbridge . & (He, became, A Player-Coach) $\rightarrow$ (neville\_southall.Q436650, occupation.P106, A Player-Coach)\\ \hline
John\_Maynard\_Keynes & After the war , Winston Churchill attempted to check the rise of Keynesian policy - making in the United Kingdom and used rhetoric critical of the mixed economy in his 1945 election campaign . & (Keynesian Policy-Making, in, The United Kingdom) $\rightarrow$ (john\_maynard\_keynes.Q9317, in, united\_kingdom.P145)\\ \hline
John\_Maynard\_Keynes & Apart from Great Britain , Keynes ' s attention was primarily focused on the United States . & (Keynes'S Attention, was, The United States) $\rightarrow$ (john\_maynard\_keynes.Q9317, was, united\_states.Q30)\\ \hline
John\_Maynard\_Keynes & John Maynard Keynes John Maynard Keynes , 1st Baron Keynes , was a British economist , whose ideas fundamentally changed the theory and practice of macroeconomics and the economic policies of governments . & (John Maynard Keynes, was, A British Economist) $\rightarrow$ (john\_maynard\_keynes.Q9317, was, united\_kingdom.P145)\\ \hline
Ernst\_Haeckel & Ernst Haeckel Ernst Heinrich Philipp August Haeckel was a German zoologist , naturalist , philosopher , physician , professor , marine biologist , and artist who discovered , described and named thousands of new species , mapped a genealogical tree relating all life forms , and coined many terms in biology , including " ecology " , " phylum " , " phylogeny " , and " Protista . " & (August Haeckel, was, A German Zoologist) $\rightarrow$ (ernst\_haeckel.Q48246, was, germany.Q183)\\ \hline
Ernst\_Haeckel & Haeckel was awarded the title of Excellency by Kaiser Wilhelm II in 1907 and the Linnean Society of London ' s prestigious Darwin - Wallace Medal in 1908 . & (Haeckel, was awarded the, Excellency) $\rightarrow$ (ernst\_haeckel.Q48246, award\_received.P166, Excellency)\\ \hline
Ernst\_Haeckel & He was also a pacifist until the First World War , when he wrote propaganda in favor of the war . & (He, was, A Pacifist) $\rightarrow$ (ernst\_haeckel.Q48246, was, A Pacifist)\\ 

==> appendices_table/unmapped_compare_kbp.tex <==
SF13\_ENG\_001 & Bashardost was born in 1965 in the southern Ghanzi province and his family migrated to Iran and then to Pakistan after successive coup and factional fighting in Afghanistan . & (Bashardost, in, The Southern Ghanzi Province) $\rightarrow$ (Ramazan Bashardost, per:stateorprovince\_of\_birth, The Southern Ghanzi Province) & -\\ \hline
SF13\_ENG\_009 & He took office in 2006 by defeating longtime incumbent Anwar Chowdhry from Pakistan, who was later barred for alleged financial corruption. & (Longtime Incumbent Anwar Chowdhry, from, Pakistan) $\rightarrow$ (Anwar Chowdhry, per:origin, Pakistan) & (Longtime Incumbent Anwar Chowdhry, from, Pakistan) $\rightarrow$ (Anwar Chowdhry, per:countries\_of\_residence, Pakistan)\\ \hline
SF13\_ENG\_012 & Gadahn , also known as Azzam the American , was born in 1978 . & (Gadahn, ,, Azzam) $\rightarrow$ (Adam Gadahn, per:alternate\_names, Azzam) & (Gadahn, also known as, Azzam) $\rightarrow$ (Adam Gadahn, per:alternate\_names, Azzam)\\ \hline
SF13\_ENG\_012 &  The message also featured several appearances of Adam Gadahn, also known as Azzam al-Amriki, an American who grew up in Riverside County and converted to Islam and joined al-Qaida.  & (Adam Gadahn, also known as, Azzam Al-Amriki) $\rightarrow$ (Adam Gadahn, per:alternate\_names, Azzam Al-Amriki) & (Adam Gadahn, also, Azzam Al-Amriki) $\rightarrow$ (Adam Gadahn, per:alternate\_names, Azzam Al-Amriki); (Adam Gadahn, ,, Azzam Al-Amriki) $\rightarrow$ (Adam Gadahn, per:alternate\_names, Azzam Al-Amriki)\\ \hline
SF13\_ENG\_014 &  Mohammed Oudeh, a former math teacher who became the mastermind of the deadly attack on Israeli athletes at the 1972 Munich Olympics, died Friday in Damascus. & (Mohammed Oudeh, ,, teacher) $\rightarrow$ (Mohammed Oudeh, per:title, teacher) & -\\ \hline
SF13\_ENG\_014 &  He settled in the West Bank town of Ramallah, but in 1999, after a trip to Jordan, he was barred by Israel from returning. & (He, in, The West Bank Town) $\rightarrow$ (Mohammed Oudeh, per:cities\_of\_residence, The West Bank Town)& (He, settled in, The West Bank Town) $\rightarrow$ (Mohammed Oudeh, per:cities\_of\_residence, The West Bank Town)\\ \hline
SF13\_ENG\_014 &  Mohammed Oudeh, a former math teacher who became the mastermind of the deadly attack on Israeli athletes at the 1972 Munich Olympics, died Friday in Damascus. & (Mohammed Oudeh, ,, A Former Math Teacher) $\rightarrow$ (Mohammed Oudeh, per:title, A Former Math Teacher) & (Mohammed Oudeh, ,, teacher) $\rightarrow$ (Mohammed Oudeh, per:title, teacher)\\ \hline
SF13\_ENG\_014 &  In later years, as a graying member of the Palestinian old guard, Oudeh, most commonly known by his guerrilla name, Abu Daoud, showed no remorse for the botched hostage taking and killings of 11 members of the Israeli Olympic team that shook the world. & (Oudeh, ,, Abu Daoud) $\rightarrow$ (Mohammed Oudeh, per:alternate\_names, Abu Daoud) & -\\ \hline
SF13\_ENG\_015 & The precise cause of death had not been determined , her sister , Elaine Philip , told The Associated Press on Sunday . & - & (Her Sister, ,, Elaine Philip) $\rightarrow$ (Lucille Clifton, per:siblings, Elaine Philip)\\ \hline
SF13\_ENG\_015 &  After her husband died in 1984, Clifton taught at the University of California at Santa Cruz before returning to Maryland in 1989. & (Clifton, of, Santa Cruz) $\rightarrow$ (Lucille Clifton, per:cities\_of\_residence, Santa Cruz) & (Clifton, taught at, the University) $\rightarrow$ (Lucille Clifton, per:employee\_or\_member\_of, the University of California)\\ \hline
SF13\_ENG\_015 &  Lucille Clifton, a National Book Award-winning poet and Pulitzer finalist, has died. & - & (Lucille Clifton, ,, poet) $\rightarrow$ (Lucille Clifton, per:title, poet)\\ \hline
SF13\_ENG\_015 &  When she was a girl, Lucille Clifton sat on her mother's lap and listened to her recite poetry. & - & (Lucille Clifton, ,, A Girl) $\rightarrow$ (Lucille Clifton, gender, A Girl) \\ \hline
SF13\_ENG\_015 &  In 1967, they moved to Baltimore, and Clifton worked in Washington for the old U.S. Office of Education. & (Clifton, worked in, old U.S. Office) $\rightarrow$ (Lucille Clifton, per:employee\_or\_member\_of, U.S. Office of Education) & (They, to, Baltimore) $\rightarrow$ (Lucille Clifton, per:cities\_of\_residence, Baltimore)\\ \hline
SF13\_ENG\_015 &  Clifton's sister, Elaine Philip, said the former poet laureate of Maryland passed away Saturday morning at Johns Hopkins University Hospital in Baltimore. & - & (Clifton'S Sister, ,, Elaine Philip) $\rightarrow$ (Lucille Clifton, per:siblings, Elaine Philip) \\ \hline
SF13\_ENG\_018 &  Harvey Pekar, the writer of comics whose autobiographical comic book series "American Splendor" chronicled his life as a filing clerk, record collector, freelance jazz critic and one of life's all-around misfits, was found dead July 12 at his home near Cleveland. & - & (Harvey Pekar, ,, writer) $\rightarrow$ (Harvey Pekar, per:title, writer)\\ \hline
SF13\_ENG\_018 &  Pekar attended what became Case Western Reserve University, served in the Navy in the late 1950s and worked a series of menial jobs before taking a 30-year jobas a filing clerk at a VA hospital in Cleveland. & - & (Pekar, what became, Case Western Reserve University) $\rightarrow$ (Harvey Pekar, per:schools\_attended, Case Western Reserve University)\\ \hline
SF13\_ENG\_025 &  Kissel, 46, of Adrian, Michigan, was convicted of drugging then bashing her husband Robert to death in a luxury Hong Kong apartment and sentenced to life in prison in September 2005. & - & (Kissel, ,, Adrian) $\rightarrow$ (Nancy Kissel, per:cities\_of\_residence, Adrian); (Kissel, ,, Michigan) $\rightarrow$ (Nancy Kissel, per:statesorprovinces\_of\_residence, Michigan)\\ \hline
SF13\_ENG\_037 & CLAUDE CHABROL , PIONEER FRENCH FILMMAKER , DIES AT 80 Joseph Berger contributed reporting from New York , and Maia de la Baume contributed from Paris . & (Claude Chabrol, ,, Pioneer French Filmmaker) $\rightarrow$ (Claude Chabrol, per:title, Pioneer French Filmmaker) & - \\ \hline
SF13\_ENG\_037 & Chabrol ' s survivors also include his third wife , Aurore Pajot , who acted as his script supervisor on nearly all of his movies from 1968 on and whom he married in 1981 ; and Pajot ' s daughter , Cecile Maistre , who was an assistant director on his films and wrote the script with him for " The Girl Cut in Two " ( 2007 ) . & (His Third Wife, ,, Aurore Pajot) $\rightarrow$ (Claude Chabrol, per:spouse, Aurore Pajot) & (Chabrol's survivors, third wife, Aurore Pajot) $\rightarrow$ (Claude Chabrol, per:spouse, Aurore Pajot)\\ \hline
SF13\_ENG\_038 &  Mercier Philip Cunningham was born in Centralia, Wash., on April 16, 1919. & - & (Mercier Philip Cunningham, was born in, Centralia) $\rightarrow$ (Merce Cunningham, was born in, Centralia); (Mercier Philip Cunningham, in, Wash.) $\rightarrow$ (Merce Cunningham, per:stateorprovince\_of\_birth, Wash.); (Mercier Philip Cunningham, in, April) $\rightarrow$ (Merce Cunningham, per:date\_of\_birth, 1919-04-16)\\ \hline
SF13\_ENG\_038 &  Cunningham's survivors include a brother, Jack Cunningham of Centralia. & - & (Cunningham'S Survivors, ,, Jack Cunningham) $\rightarrow$ (Merce Cunningham, per:siblings, Jack Cunningham)\\ \hline
SF13\_ENG\_041 & By the time Hewitt was 6, his family was living in New Rochelle, N.Y.  & - & (Hewitt, in, New Rochelle) $\rightarrow$ (Don Hewitt, per:cities\_of\_residence, New Rochelle)\\ \hline
SF13\_ENG\_041 &  He is survived by his third wife, former television news correspondent Marilyn Berger; his sons, Steven and Jeffrey; his daughter, Lisa Cassara; his stepdaughter, Jilian Childers Hewitt, whom Hewitt adopted; and three grandchildren. & - & (Hewitt, ,, Jilian Childers Hewitt) $\rightarrow$ (Don Hewitt, per:children, Jilian Childers Hewitt)\\ \hline
SF13\_ENG\_044 & Dominick Dunne , a novelist and journalist who chronicled true - crime tales of the rich and infamous , including O . J . Simpson and Claus von Bulow , and in turn became a celebrity in his own right , died of bladder cancer Aug . 26 at his home in New York City . & (Dominick Dunne, ,, A Novelist) $\rightarrow$ (Dominick Dunne, per:title, A Novelist) & (Dunne, ,, novelist) $\rightarrow$ (Dominick Dunne, per:title, novelist)\\ \hline
SF13\_ENG\_044 & Dunne and his wife , Ellen Griffin Dunne , known as Lenny , were married in 1954 . & (His Wife, ,, Ellen Griffin Dunne) $\rightarrow$ (Dominick Dunne, per:spouse, Ellen Griffin Dunne) & (Dunne, and, Ellen Griffin Dunne) $\rightarrow$ (Dominick Dunne, per:spouse, Ellen Griffin Dunne)\\ \hline
SF13\_ENG\_044 &  Dunne was born in 1925 in Hartford, Connecticut, to a wealthy Roman Catholic family and grew up in some of the same social circles as the Kennedys. & (Dunne, was born in 1925 in, Connecticut) $\rightarrow$ (Dominick Dunne, per:stateorprovince\_of\_birth, Connecticut) & (Dunne, was born in 1925 in, Connecticut) $\rightarrow$ (Dominick Dunne, per:stateorprovince\_of\_birth, Connecticut)\\ \hline
SF13\_ENG\_044 &  Dunne was part of a famous family that also included his brother, novelist and screenwriter John Gregory Dunne; his brother's wife, author Joan Didion; and his son, Griffin. & - & (His Brother, ,, Novelist) $\rightarrow$ (His brother, per:title, Novelist)\\ \hline
SF13\_ENG\_047 &  The women were accompanied by Reyna Luisa Tamayo, the mother of political prisoner Orlando Zapata, who died at age 42 in a hunger strike February 23 to protest prison conditions. & (Political Prisoner Orlando Zapata, ,, Reyna Luisa Tamayo) $\rightarrow$ (Orlando Zapata, per:children, Reyna Luisa Tamayo) & (Political Prisoner Orlando Zapata, ,, Reyna Luisa Tamayo) $\rightarrow$ (Orlando Zapata, per:children, Reyna Luisa Tamayo) \\ \hline
SF13\_ENG\_049 & A professor emeritus at Yale University , Mandelbrot was born in Poland but as a child moved with his family to France where he was educated . & (Mandelbrot, ,, Yale University) $\rightarrow$ (Benoit Mandelbrot, per:employee\_or\_member\_of, Yale University) & (Mandelbrot, was born in, Poland) $\rightarrow$ (Benoit Mandelbrot, per:country\_of\_birth, Poland)\\ \hline
SF13\_ENG\_058 & Access Industries , a privately held company founded in 1986 by Len Blavatnik , has a diverse portfolio of investments in industry , real estate , media and telecommunications . & (Access Industries, ,, A Privately Held Company) $\rightarrow$ (Access Industries, properties, A Privately Held Company) & (Access Industries, founded in 1986 by, Len Blavatnik) $\rightarrow$ (Access Industries, org:founded\_by, Len Blavatnik)\\ \hline
SF13\_ENG\_061 &  InterContinental Hotels Group, owners of Holiday Inn Worldwide, has been ordered by a court to pay \$25 million in damages to a franchisee for fraud. & (Intercontinental Hotels Group, ,, Holiday Inn Worldwide) $\rightarrow$ (InterContinental Hotels Group, org:parents, Holiday Inn Worldwide) & (Intercontinental Hotels Group, ,, Holiday Inn Worldwide) $\rightarrow$ (InterContinental Hotels Group, org:parents, Holiday Inn Worldwide)\\ \hline
SF13\_ENG\_079 &  Water and its links to development, peace and conflict were key words in the annual sessions, Anders Berntell, executive director of Stockholm International Water Institute (SIWI), said in his opening address. & (Stockholm International, director, Anders Berntell) $\rightarrow$ (Stockholm International Water Institute, per:top\_members\_or\_employees, Anders Berntell) &-\\ \hline
SF13\_ENG\_079 &  Water and its links to development, peace and conflict were key words in the annual sessions, Anders Berntell, executive director of Stockholm International Water Institute (SIWI), said in his opening address. & (Stockholm International, , executive director, Anders Berntell) $\rightarrow$ (Stockholm International Water Institute, per:top\_members\_or\_employees, Anders Berntell) & (Stockholm International, , executive director, Anders Berntell) $\rightarrow$ (Stockholm International Water Institute, per:top\_members\_or\_employees, Anders Berntell) \\ \hline
SF13\_ENG\_090 &  ECO member countries include Afghanistan, Azerbaijan, Iran, Kazakhstan, Kyrgyzstan, Pakistan, Tajikistan, Turkey, Turkmenistan and Uzbekistan. & (Eco Member Countries, include, Azerbaijan)  $\rightarrow$ (Economic Cooperation Organization, org:members, Azerbaijan) & (Eco Member Countries, ,, Azerbaijan) $\rightarrow$ (Economic Cooperation Organization, org:members, Azerbaijan)\\ \hline
SF13\_ENG\_096 &  Freedom was founded in the 1930s by R.C. Hoiles and is still majority owned by the Hoiles family. & (Freedom, was founded in, The 1930S)$\rightarrow$ (Freedom Communications, org:date\_founded, 1930-XX-XX) & (Freedom, was founded in, The 1930S)$\rightarrow$ (Freedom Communications, org:date\_founded, 1930-XX-XX) \\ \hline
SF13\_ENG\_096 &  A phone message left Sunday at Freedom's Irvine, California, headquarters was not immediately returned. & - & (Freedom'S Irvine, ,, California)$\rightarrow$ (Freedom Communications, org:stateorprovince\_of\_headquarters, California)\\ \hline
SF13\_ENG\_097 &  STX Finland is part of the international STX Europe Group, with shipyards in Brazil, Norway, France, Romania and Vietnam. & (Stx Finland, of, The International Stx Europe Group)$\rightarrow$ (STX Finland, org:subsidaries, The International Stx Europe Group) & (Stx Finland, of, The International Stx Europe Group)$\rightarrow$ (STX Finland, org:subsidaries, The International Stx Europe Group) \\

==> appendices_table/unmapped_compare_wikidata.tex <==
Nick\_Aldis & He was also a co - presenter of " Britain ' s Strongest Man " on Challenge TV in the United Kingdom . & (Challenge Tv, in, The United Kingdom) $\rightarrow$ (Challenge TV, in, united\_kingdom.Q145) & -\\ \hline
Douglas\_Bader & Group Captain Sir Douglas Robert Steuart Bader, was a Royal Air Force flying ace during the Second World War. & - & (Douglas Bader  Group Captain Sir Douglas Robert Steuart Bader, was, A Royal Air Force Flying Ace) $\rightarrow$ (douglas\_bader.Q348780, was, flying\_ace.Q222982)\\ \hline
Douglas\_Bader & At the age of two , Bader joined his parents in India for a year . & (His Parents, in, India) $\rightarrow$ (douglas\_bader.Q348780, in, india.Q668) & -\\ \hline
Douglas\_Bader & On 2 July 1941 he was awarded the bar to his DSO. & (He, was awarded the bar, his DSO) $\rightarrow$ (douglas\_bader.Q348780, was awarded the bar, distinguished\_service\_order.Q615838) & (He, was awarded the bar to, his DSO) $\rightarrow$ (douglas\_bader.Q348780, was awarded the bar to, distinguished\_service\_order.Q615838) \\ \hline
Helen\_Storrow & His father , also named James Jackson Storrow , was a prominent attorney , whose clients included Alexander Graham Bell and the government of Venezuela ; his mother , Ann Maria Perry , was the grandchild of naval hero Commodore Oliver Hazard Perry , and a distant cousin of President Thomas Jefferson . & (His Father, was, A Prominent Attorney) $\rightarrow$ (His Father, occupation.P106, lawyer.Q40348) & (His Father, was, A Prominent Attorney) $\rightarrow$ (His Father, occupation.P106, lawyer.Q40348)\\ \hline
Helen\_Storrow & Helen Osborne Storrow was a prominent American philanthropist, early Girl Scout leader, and chair of the World Committee of the World Association of Girl Guides and Girl Scouts          for eight years. & (Helen Osborne Storrow, was, A Prominent American Philanthropist) $\rightarrow$ (helen\_storrow.Q5703224, was, united\_states.Q30) & (Helen Osborne Storrow, was, A Prominent American Philanthropist) $\rightarrow$ (helen\_storrow.Q5703224, was, united\_states.Q30)\\ \hline
Jacob\_Van\_Ruisdael & Ruisdael lived and worked in Amsterdam for the rest of his life. & - & (Ruisdael, lived, Amsterdam) $\rightarrow$ (jacob\_van\_ruisdael.Q213612, lived, amsterdam.Q727); (Ruisdael, lived and worked in, Amsterdam) $\rightarrow$ (jacob\_van\_ruisdael.Q213612, lived and worked in, amsterdam.Q727)\\ \hline
Jacob\_Van\_Ruisdael & His cousin Jacob was a registered Mennonite in Amsterdam . & (His Cousin, was, A Registered Mennonite) $\rightarrow$ (His Cousin, was, A Registered Mennonite) & - \\ \hline
Jacob\_Van\_Ruisdael & He appears to have been strongly influenced by other contemporary local Haarlem landscapists , most notably Cornelis Vroom and Allaert van Everdingen . & (He, have been strongly influenced by, landscape painting) $\rightarrow$ (jacob\_van\_ruisdael.Q213612, have been strongly influenced by, landscape\_art.Q191163) & -\\ \hline
Liaquat\_Ali\_Khan & Liaquat Ali Khan was educated at the Aligarh Muslim University in India, and then at Oxford University in the United Kingdom. & (Liaquat Ali Khan, in, India) $\rightarrow$ (liaquat\_ali\_khan.Q295713, in, india.Q668) & (Liaquat Ali Khan, was educated at, The Aligarh Muslim University) $\rightarrow$ (liaquat\_ali\_khan.Q295713, was educated at, aligarh\_muslim\_university.Q196544)\\ \hline
Liaquat\_Ali\_Khan & After the death of his father in 1919, Ali Khan, with British Government awarding the grants and scholarship, went to England, attending Oxford University's Exeter College to pursue his higher education. & - & (His Higher Education, pursue, Oxford University'S Exeter College) $\rightarrow$ (liaquat\_ali\_khan.Q295713, pursue, university\_of\_oxford.Q34433)\\ \hline
Liaquat\_Ali\_Khan & In 1940, Khan was made the deputy leader of the Muslim League Parliamentary party. & - & (Khan, was made the deputy leader of, The Muslim League Parliamentary Party) $\rightarrow$ (liaquat\_ali\_khan.Q295713, deputy leader, all-india\_muslim\_league.Q223898)\\ \hline
Pauline\_Baynes &   When Baynes's father retired, he left India and returned to England, settling with Baynes's mother in a house close to Baynes's own near Farnham in southwest Surrey. & - & (He, left, India) $\rightarrow$ (pauline\_baynes.Q101951, left, india.Q668)\\ \hline
Pauline\_Baynes &   Baynes began her education at a convent school. & (Her Education, at, A Convent School) $\rightarrow$ (pauline\_baynes.Q101951, at, catholic\_school.Q1138671) & (Her Education, at, A Convent School) $\rightarrow$ (pauline\_baynes.Q101951, at, catholic\_school.Q1138671)\\ \hline
Pauline\_Baynes & Her most vivid recollection of their New Year's Eve lunch at Magdalen College was of his gleefully picking nuts out of a bowl of Brussels sprouts. & (Their New Year'S Eve Lunch, at, Magdalen College) $\rightarrow$ (pauline\_baynes.Q101951, at, magdalen\_college,\_oxford.Q81162) & (Their New Year'S Eve Lunch, at, Magdalen College) $\rightarrow$ (pauline\_baynes.Q101951, at, magdalen\_college,\_oxford.Q81162)\\ \hline
Pauline\_Baynes & She was not a diligent student, frittering away her time on \"coffee and parties\", and she left the Slade without a qualification, But she did achieve the distinction, one shared with her sister, of exhibiting at the Royal Academy of Arts in 1939, In 1940, a year into World War II, both Baynes sisters joined the Women's Voluntary Service. & - & (She, without a qualification, The Slade) $\rightarrow$ (pauline\_baynes.Q101951, without a qualification, slade\_school\_of\_fine\_art.Q1399299)\\ \hline
Pauline\_Baynes & By the time that she left , she had already formed the ambition of becoming an illustrator . & (She, formed the ambition of becoming, An Illustrator) $\rightarrow$ (pauline\_baynes.Q101951, formed the ambition of becoming, illustrator.Q644687) & -\\ \hline
Thor\_Heyerdahl & His theories rarely won any scientific acceptance, whereas Heyerdahl himself rejected all scientific criticism and concentrated on publishing his theories in popular books aimed at the general public. & - & (His Theories, at, The General Public) $\rightarrow$ (thor\_heyerdahl.Q133622, at, general\_public)\\ \hline
Thor\_Heyerdahl & He was an atheist . & (He, was, An Atheist) $\rightarrow$ (thor\_heyerdahl.Q133622, was, An Atheist) & (He, was, An Atheist) $\rightarrow$ (thor\_heyerdahl.Q133622, was, An Atheist)\\ \hline
Thor\_Heyerdahl & He is buried in the garden of the family home in Colla Micheri . & (He, is buried, Colla Micheri) $\rightarrow$ (thor\_heyerdahl.Q133622, is buried, colla\_micheri.Q3647771) & -\\ \hline
Neville\_Southall &   As a teenager, Southall had unsuccessful trials at Wrexham, Crewe Alexandra and Bolton Wanderers. & - & (Southall, at, Wrexham) $\rightarrow$ (neville\_southall.Q436650, at, wrexham\_a.f.c..Q18529); (Southall, at, Crewe Alexandra) $\rightarrow$ (neville\_southall.Q436650, at, crewe\_alexandra\_f.c..Q19587)\\ \hline
Neville\_Southall & He moved on to Cheshire County League club Winsford United at the age of 20 . & (He, to, Cheshire County League Club Winsford United) $\rightarrow$ (neville\_southall.Q436650, to, winsford\_united\_f.c..Q5213266) & -\\ \hline
Neville\_Southall & He later became a player - coach at York City , Rhyl , Shrewsbury Town and Dagenham \& Redbridge . & (He, became, A Player-Coach) $\rightarrow$ (neville\_southall.Q436650, occupation.P106, A Player-Coach) & -\\ \hline
John\_Maynard\_Keynes &   In January 1889 at the age of five and a half, Keynes started at the kindergarten of the Perse School for Girls for five mornings a week. & - & (Keynes, at, The Perse School) $\rightarrow$ (john\_maynard\_keynes.Q9317, at, the\_perse\_school.Q7756751)\\ \hline
John\_Maynard\_Keynes & In January 1892, at eight and a half, he started as a day pupil at St Faith's preparatory school. & - & (He, at, St Faith'S Preparatory School) $\rightarrow$ (john\_maynard\_keynes.Q9317, at, st\_faith's\_school.Q7593056)\\ \hline
John\_Maynard\_Keynes & After the war , Winston Churchill attempted to check the rise of Keynesian policy - making in the United Kingdom and used rhetoric critical of the mixed economy in his 1945 election campaign . & (Keynesian Policy-Making, in, The United Kingdom) $\rightarrow$ (john\_maynard\_keynes.Q9317, in, united\_kingdom.P145) & -\\ \hline
John\_Maynard\_Keynes & Keynes was a lifelong member of the Liberal Party, which until the 1920s had been one of the two main political parties in the United Kingdom, and as late as 1916 had often been the dominant power in government. & - & (Keynes, was a lifelong member of, The liberal party) $\rightarrow$ (john\_maynard\_keynes.Q9317, was a lifelong member of, liberal\_party\_(uk).Q622441) \\ \hline
Ernst\_Haeckel & Ernst Haeckel Ernst Heinrich Philipp August Haeckel was a German zoologist , naturalist , philosopher , physician , professor , marine biologist , and artist who discovered , described and named thousands of new species , mapped a genealogical tree relating all life forms , and coined many terms in biology , including " ecology " , " phylum " , " phylogeny " , and " Protista . " & (August Haeckel, was, A German Zoologist) $\rightarrow$ (ernst\_haeckel.Q48246, was, germany.Q183) & -\\ \hline
Ernst\_Haeckel & Ernst Haeckel was born on 16 February 1834, in Potsdam. & - & (Haeckel, was born on 17 February 1834, in, Potsdam) $\rightarrow$ (ernst\_haeckel.Q48246, was born on 17 February 1834, in, potsdam.Q1711) \\ \hline
Ernst\_Haeckel &   Haeckel was awarded the title of Excellency by Kaiser Wilhelm II in 1907 and the Linnean Society of London's prestigious Darwin-Wallace Medal in 1908. & (Haeckel, was awarded the, Excellency) $\rightarrow$ (ernst\_haeckel.Q48246, award\_received.P166, Excellency) & (Haeckel, was awarded the, Excellency) $\rightarrow$ (ernst\_haeckel.Q48246, award\_received.P166, Excellency)\\ \hline
Ernst\_Haeckel & He was also a pacifist until the First World War, when he wrote propaganda in favor of the war. & (He, was, A Pacifist) $\rightarrow$ (ernst\_haeckel.Q48246, was, A Pacifist)& (He, was, A Pacifist) $\rightarrow$ (ernst\_haeckel.Q48246, was, A Pacifist)\\

==> appendices_table/unmapped_gpt2xl_kbp.tex <==
SF13\_ENG\_009 & He took office in 2006 by defeating longtime incumbent Anwar Chowdhry from Pakistan, who was later barred for alleged financial corruption. & (Longtime Incumbent Anwar Chowdhry, from, Pakistan) $\rightarrow$ (Anwar Chowdhry, per:countries\_of\_residence, Pakistan)\\ \hline
SF13\_ENG\_012 &  The message also featured several appearances of Adam Gadahn, also known as Azzam al-Amriki, an American who grew up in Riverside County and converted to Islam and joined al-Qaida. & (Adam Gadahn, also, Azzam Al-Amriki) $\rightarrow$ (Adam Gadahn, per:alternate\_names, Azzam Al-Amriki); (Adam Gadahn, ,, Azzam Al-Amriki) $\rightarrow$ (Adam Gadahn, ,, Azzam Al-Amriki)\\ \hline
SF13\_ENG\_014 &  Mohammed Oudeh, a former math teacher who became the mastermind of the deadly attack on Israeli athletes at the 1972 Munich Olympics, died Friday in Damascus. & (Mohammed Oudeh, ,, teacher) $\rightarrow$ (Mohammed Oudeh, per:title, teacher)\\ \hline
SF13\_ENG\_014 &  He settled in the West Bank town of Ramallah, but in 1999, after a trip to Jordan, he was barred by Israel from returning. & (He, in, The West Bank Town) $\rightarrow$ (Mohammed Oudeh, per:cities\_of\_residence, The West Bank Town)\\ \hline
SF13\_ENG\_014 &  Mohammed Oudeh, a former math teacher who became the mastermind of the deadly attack on Israeli athletes at the 1972 Munich Olympics, died Friday in Damascus. & (Mohammed Oudeh, ,, A Former Math Teacher) $\rightarrow$ (Mohammed Oudeh, per:title, A Former Math Teacher)\\ \hline
SF13\_ENG\_014 &  In later years, as a graying member of the Palestinian old guard, Oudeh, most commonly known by his guerrilla name, Abu Daoud, showed no remorse for the botched hostage taking and killings of 11 members of the Israeli Olympic team that shook the world. & (Oudeh, ,, Abu Daoud) $\rightarrow$ (Mohammed Oudeh, per:alternate\_names, Abu Daoud)\\ \hline
SF13\_ENG\_015 &  After her husband died in 1984, Clifton taught at the University of California at Santa Cruz before returning to Maryland in 1989. & (Clifton, of, Santa Cruz) $\rightarrow$ (Lucille Clifton, per:cities\_of\_residence, Santa Cruz)\\ \hline
SF13\_ENG\_015 &  Lucille Clifton, a National Book Award-winning poet and Pulitzer finalist, has died. & (Lucille Clifton, ,, poet) $\rightarrow$ (Lucille Clifton, per:title, poet)\\ \hline
SF13\_ENG\_015 &  When she was a girl, Lucille Clifton sat on her mother's lap and listened to her recite poetry. & (Lucille Clifton, ,, A Girl) $\rightarrow$ (Lucille Clifton, gender, A Girl)\\ \hline
SF13\_ENG\_015 &  In 1967, they moved to Baltimore, and Clifton worked in Washington for the old U.S. Office of Education. & (They, to, Baltimore) $\rightarrow$ (Lucille Clifton, per:cities\_of\_residence, Baltimore)\\ \hline
SF13\_ENG\_015 &  Clifton's sister, Elaine Philip, said the former poet laureate of Maryland passed away Saturday morning at Johns Hopkins University Hospital in Baltimore. & (Clifton'S Sister, ,, Elaine Philip) $\rightarrow$ (Lucille Clifton, per:siblings, Elaine Philip)\\ \hline
SF13\_ENG\_018 &  Harvey Pekar, the writer of comics whose autobiographical comic book series "American Splendor" chronicled his life as a filing clerk, record collector, freelance jazz critic and one of life's all-around misfits, was found dead July 12 at his home near Cleveland. & (Harvey Pekar, ,, writer) $\rightarrow$ (Harvey Pekar, per:title, writer)\\ \hline
SF13\_ENG\_018 &  Pekar attended what became Case Western Reserve University, served in the Navy in the late 1950s and worked a series of menial jobs before taking a 30-year jobas a filing clerk at a VA hospital in Cleveland. & (Pekar, what became, Case Western Reserve University) $\rightarrow$ (Harvey Pekar, per:schools\_attended, Case Western Reserve University)\\ \hline
SF13\_ENG\_025 &  Kissel, 46, of Adrian, Michigan, was convicted of drugging then bashing her husband Robert to death in a luxury Hong Kong apartment and sentenced to life in prison in September 2005. & (Kissel, ,, Adrian) $\rightarrow$ (Nancy Kissel, per:cities\_of\_residence, Adrian); (Kissel, ,, Michigan) $\rightarrow$ (Nancy Kissel, per:statesorprovinces\_of\_residence, Michigan)\\ \hline
SF13\_ENG\_038 &  Mercier Philip Cunningham was born in Centralia, Wash., on April 16, 1919. & (Mercier Philip Cunningham, was born in, Centralia) $\rightarrow$ (Merce Cunningham, was born in, Centralia); (Mercier Philip Cunningham, in, Wash.) $\rightarrow$ (Merce Cunningham, per:stateorprovince\_of\_birth, Wash.); (Mercier Philip Cunningham, in, April) $\rightarrow$ (Merce Cunningham, per:date\_of\_birth, 1919-04-16)\\ \hline
SF13\_ENG\_038 &  Cunningham's survivors include a brother, Jack Cunningham of Centralia. & (Cunningham'S Survivors, ,, Jack Cunningham) $\rightarrow$ (Merce Cunningham, per:siblings, Jack Cunningham)\\ \hline
SF13\_ENG\_041 & By the time Hewitt was 6, his family was living in New Rochelle, N.Y.  & (Hewitt, in, New Rochelle) $\rightarrow$ (Don Hewitt, per:cities\_of\_residence, New Rochelle)\\ \hline
SF13\_ENG\_041 &  He is survived by his third wife, former television news correspondent Marilyn Berger; his sons, Steven and Jeffrey; his daughter, Lisa Cassara; his stepdaughter, Jilian Childers Hewitt, whom Hewitt adopted; and three grandchildren. & (Hewitt, ,, Jilian Childers Hewitt) $\rightarrow$ (Don Hewitt, per:children, Jilian Childers Hewitt)\\ \hline
SF13\_ENG\_044 &  Dunne was born in 1925 in Hartford, Connecticut, to a wealthy Roman Catholic family and grew up in some of the same social circles as the Kennedys. & (Dunne, was born in 1925 in, Connecticut) $\rightarrow$ (Dominick Dunne, per:stateorprovince\_of\_birth, Connecticut)\\ \hline
SF13\_ENG\_044 &  Dunne was part of a famous family that also included his brother, novelist and screenwriter John Gregory Dunne; his brother's wife, author Joan Didion; and his son, Griffin. & (His Brother, ,, Novelist) $\rightarrow$ (His brother, per:title, Novelist)\\ \hline
SF13\_ENG\_044 &  Dunne and his wife, Ellen Griffin Dunne, known as Lenny, were married in 1954. & (Dunne, and, Ellen Griffin Dunne) $\rightarrow$ (Dominick Dunne, per:spouse, Ellen Griffin Dunne)\\ \hline
SF13\_ENG\_047 &  The women were accompanied by Reyna Luisa Tamayo, the mother of political prisoner Orlando Zapata, who died at age 42 in a hunger strike February 23 to protest prison conditions. & (Political Prisoner Orlando Zapata, ,, Reyna Luisa Tamayo) $\rightarrow$ (Orlando Zapata, per:children, Reyna Luisa Tamayo)\\ \hline
SF13\_ENG\_061 &  InterContinental Hotels Group, owners of Holiday Inn Worldwide, has been ordered by a court to pay \$25 million in damages to a franchisee for fraud. & (Intercontinental Hotels Group, ,, Holiday Inn Worldwide) $\rightarrow$ (InterContinental Hotels Group, org:parents, Holiday Inn Worldwide)\\ \hline
SF13\_ENG\_079 &  Water and its links to development, peace and conflict were key words in the annual sessions, Anders Berntell, executive director of Stockholm International Water Institute (SIWI), said in his opening address. & (Stockholm International, director, Anders Berntell) $\rightarrow$ (Stockholm International Water Institute, per:top\_members\_or\_employees, Anders Berntell); (Stockholm International, , executive director, Anders Berntell) $\rightarrow$ (Stockholm International Water Institute, per:top\_members\_or\_employees, Anders Berntell)\\ \hline
SF13\_ENG\_090 &  ECO member countries include Afghanistan, Azerbaijan, Iran, Kazakhstan, Kyrgyzstan, Pakistan, Tajikistan, Turkey, Turkmenistan and Uzbekistan. & (Eco Member Countries, ,, Azerbaijan) $\rightarrow$ (Economic Cooperation Organization, org:members, Azerbaijan)\\ \hline
SF13\_ENG\_096 &  A phone message left Sunday at Freedom's Irvine, California, headquarters was not immediately returned. & (Freedom'S Irvine, ,, California)$\rightarrow$ (Freedom Communications, org:stateorprovince\_of\_headquarters, California)\\ \hline
SF13\_ENG\_097 &  STX Finland is part of the international STX Europe Group, with shipyards in Brazil, Norway, France, Romania and Vietnam. & (Stx Finland, of, The International Stx Europe Group)$\rightarrow$ (STX Finland, org:subsidaries, The International Stx Europe Group)\\

==> appendices_table/unmapped_gpt2xl_wikidata.tex <==
Douglas\_Bader & He left St Edward's in early 1928, aged 18. & (He, left, St Edward) $\rightarrow$ (douglas\_bader.Q348780, left, st\_edward's\_school,\_oxford.Q128260)\\ \hline
Douglas\_Bader & Group Captain Sir Douglas Robert Steuart Bader, was a Royal Air Force flying ace during the Second World War. & (Douglas Bader  Group Captain Sir Douglas Robert Steuart Bader, was, A Royal Air Force Flying Ace) $\rightarrow$ (douglas\_bader.Q348780, was, flying\_ace.Q222982)\\ \hline
Douglas\_Bader & On 2 July 1941 he was awarded the bar to his DSO. & (He, was awarded the bar to, his DSO) $\rightarrow$ (douglas\_bader.Q348780, was awarded the bar to, distinguished\_service\_order.Q615838) \\ \hline
Helen\_Storrow & His father, also named James Jackson Storrow, was a prominent attorney, whose clients included Alexander Graham Bell and the government of Venezuela; his mother, Ann Maria Perry, was the grandchild of naval hero Commodore Oliver Hazard Perry, and a distant cousin of President Thomas Jefferson. & (His Father, was, A Prominent Attorney) $\rightarrow$ (His Father, occupation.P106, lawyer.Q40348)\\ \hline
Helen\_Storrow & Helen Osborne Storrow was a prominent American philanthropist, early Girl Scout leader, and chair of the World Committee of the World Association of Girl Guides and Girl Scouts          for eight years. & (Helen Osborne Storrow, was, A Prominent American Philanthropist) $\rightarrow$ (helen\_storrow.Q5703224, was, united\_states.Q30)\\ \hline
Jacob\_Van\_Ruisdael & Ruisdael lived and worked in Amsterdam for the rest of his life. & (Ruisdael, lived, Amsterdam) $\rightarrow$ (jacob\_van\_ruisdael.Q213612, lived, amsterdam.Q727); (Ruisdael, lived and worked in, Amsterdam) $\rightarrow$ (jacob\_van\_ruisdael.Q213612, lived and worked in, amsterdam.Q727)\\ \hline
Liaquat\_Ali\_Khan & Liaquat Ali Khan was educated at the Aligarh Muslim University in India, and then at Oxford University in the United Kingdom. & (Liaquat Ali Khan, was educated at, The Aligarh Muslim University) $\rightarrow$ (liaquat\_ali\_khan.Q295713, was educated at, aligarh\_muslim\_university.Q196544)\\ \hline
Liaquat\_Ali\_Khan & After the death of his father in 1919, Ali Khan, with British Government awarding the grants and scholarship, went to England, attending Oxford University's Exeter College to pursue his higher education. & (His Higher Education, pursue, Oxford University'S Exeter College) $\rightarrow$ (liaquat\_ali\_khan.Q295713, pursue, university\_of\_oxford.Q34433)\\ \hline
Liaquat\_Ali\_Khan & In 1940, Khan was made the deputy leader of the Muslim League Parliamentary party. & (Khan, was made the deputy leader of, The Muslim League Parliamentary Party) $\rightarrow$ (liaquat\_ali\_khan.Q295713, deputy leader, all-india\_muslim\_league.Q223898)\\ \hline
Pauline\_Baynes &   When Baynes's father retired, he left India and returned to England, settling with Baynes's mother in a house close to Baynes's own near Farnham in southwest Surrey. & (He, left, India) $\rightarrow$ (pauline\_baynes.Q101951, left, india.Q668)\\ \hline
Pauline\_Baynes &   Baynes began her education at a convent school. & (Her Education, at, A Convent School) $\rightarrow$ (pauline\_baynes.Q101951, at, catholic\_school.Q1138671)\\ \hline
Pauline\_Baynes & Her most vivid recollection of their New Year's Eve lunch at Magdalen College was of his gleefully picking nuts out of a bowl of Brussels sprouts. & (Their New Year'S Eve Lunch, at, Magdalen College) $\rightarrow$ (pauline\_baynes.Q101951, at, magdalen\_college,\_oxford.Q81162)\\ \hline
Pauline\_Baynes & She was not a diligent student, frittering away her time on \"coffee and parties\", and she left the Slade without a qualification, But she did achieve the distinction, one shared with her sister, of exhibiting at the Royal Academy of Arts in 1939. In 1940, a year into World War II, both Baynes sisters joined the Women's Voluntary Service. & (She, without a qualification, The Slade) $\rightarrow$ (pauline\_baynes.Q101951, without a qualification, slade\_school\_of\_fine\_art.Q1399299)\\ \hline
Thor\_Heyerdahl & His theories rarely won any scientific acceptance, whereas Heyerdahl himself rejected all scientific criticism and concentrated on publishing his theories in popular books aimed at the general public. & (His Theories, at, The General Public) $\rightarrow$ (thor\_heyerdahl.Q133622, at, general\_public)\\ \hline
Thor\_Heyerdahl & He was an atheist. & (He, was, An Atheist) $\rightarrow$ (thor\_heyerdahl.Q133622, was, An Atheist)\\ \hline
Neville\_Southall &   As a teenager, Southall had unsuccessful trials at Wrexham, Crewe Alexandra and Bolton Wanderers. & (Southall, at, Wrexham) $\rightarrow$ (neville\_southall.Q436650, at, wrexham\_a.f.c..Q18529); (Southall, at, Crewe Alexandra) $\rightarrow$ (neville\_southall.Q436650, at, crewe\_alexandra\_f.c..Q19587)\\ \hline
John\_Maynard\_Keynes & John Maynard Keynes, 1st Baron Keynes, was a British economist, whose ideas fundamentally changed the theory and practice of macroeconomics and the economic policies of governments. & (John Maynard Keynes, was, A British Economist) $\rightarrow$ (john\_maynard\_keynes.Q9317, was, united\_kingdom.Q145)\\ \hline
John\_Maynard\_Keynes &   In January 1889 at the age of five and a half, Keynes started at the kindergarten of the Perse School for Girls for five mornings a week. & (Keynes, at, The Perse School) $\rightarrow$ (john\_maynard\_keynes.Q9317, at, the\_perse\_school.Q7756751)\\ \hline
John\_Maynard\_Keynes & In January 1892, at eight and a half, he started as a day pupil at St Faith's preparatory school. & (He, at, St Faith'S Preparatory School) $\rightarrow$ (john\_maynard\_keynes.Q9317, at, st\_faith's\_school.Q7593056)\\ \hline
John\_Maynard\_Keynes & Keynes was a lifelong member of the Liberal Party, which until the 1920s had been one of the two main political parties in the United Kingdom, and as late as 1916 had often been the dominant power in government. & (Keynes, was a lifelong member of, The liberal party) $\rightarrow$ (john\_maynard\_keynes.Q9317, was a lifelong member of, liberal\_party\_(uk).Q622441) \\ \hline
Ernst\_Haeckel &   Haeckel was awarded the title of Excellency by Kaiser Wilhelm II in 1907 and the Linnean Society of London's prestigious Darwin-Wallace Medal in 1908. & (Haeckel, was awarded the, Excellency) $\rightarrow$ (ernst\_haeckel.Q48246, award\_received.P166, Excellency)\\ \hline
Ernst\_Haeckel & He was also a pacifist until the First World War, when he wrote propaganda in favor of the war. & (He, was, A Pacifist) $\rightarrow$ (ernst\_haeckel.Q48246, was, A Pacifist)\\ \hline
Ernst\_Haeckel & He was also a social Darwinist who believed that "survival of the fittest" was a natural law, and that struggle led to improvement of the race. & (He, was, A Social Darwinist) $\rightarrow$ (ernst\_haeckel.Q48246, was, A Social Darwinist)\\ \hline
Ernst\_Haeckel & Ernst Haeckel was born on 16 February 1834, in Potsdam. & (Haeckel, was born on 17 February 1834, in, Potsdam) $\rightarrow$ (ernst\_haeckel.Q48246, was born on 17 February 1834, in, potsdam.Q1711) \\

==> misc.tex <==
% the benchmark mainly focuses on testing relations that appear in the pre-training data. For example, BERT has English Wikipedia as a part of its pre-training data, and the LAMA benchmark mostly contains relational facts derived from Wikipedia. 
%  and models are only evaluated against the gold label, and only ``birthplace'' is used to report evaluation metrics. 

% We confirm that pre-trained LMs have stored the general in-domain knowledge, even outperforming state-of-the-art open information extraction systems. We also show that the pre-trained LMs surprisingly contain a considerable amount of out-of-domain factual knowledge. Our knowledge benchmark consists of large-scale in-domain and out-of-domain datasets. For instance, our in-domain dataset is built based on Wikidata and has 1,156 relations and more than 27 million facts. To enable such large-scale evaluation, our evaluation framework involves an efficient knowledge calibration module that collects general knowledge in triple format using model parameters according to the textual corpus, and an alignment module that maps triples to facts in knowledge graphs for quantitative evaluation, as shown in Figure~\ref{fig:overview}. To the best of our knowledge, this is the first attempt on evaluating general relational knowledge in pre-trained LMs. 
    % We enable the large-scale evaluation via efficiently calibrating the relational knowledge in triple format using parameters of pre-trained LMs and aligning triples to facts in existing knowledge graphs. This helps researchers explicitly understand what the language models learn through enhanced model transparency. 
    % \item We show that pre-trained LMs have stored more accurate general knowledge compared to manually-created open information extractors. The reach of this result suggests that pre-trained LMs are alternative knowledge containers other than traditional knowledge graphs.

% In order to calculate the scores, we need to align the system extractions to the oracle facts. For example, to evaluate the  performance, we should be able to map a triple output {\sl (Dylan, is, songwriter)} to the oracle {\sl (Bob\_Dylan.Q392, occupation.P106, Songwriter.Q753110)} in Wikidata. It is infeasible to manually build the map, we instead leverage automated methods.

% For evaluation, we follow  to map the triples to TAC KBP KG facts. 

% \subsubsection{Wikidata-OIE}
% Motivated by this, we design a similar map function for  evaluation. By doing so, we enable quantitatively measuring the triples with oracle facts in both  and  KGs. Formally, to map a triple $(h, r, t)$ to a oracle fact $(h_k, r_k, t_k)$ of the  KG (Wikidata), the function first maps both entities $h, t$ to $h_k, t_k$, then maps the relation $r$ to $r_k$. 
% \begin{itemize}[leftmargin=*]
%     \item Entity linking. We adapt an unsupervised entity linker based on a mention-to-entity dictionary~\citep{spitkovsky2012cross} to link the entities for scalability consideration. Besides, contextual information is crucial to link the entities correctly, we use the word embedding of the context to disambiguate the entities, which means we only link the entities with high contextual similarities based on the word embedding. At test time, we adopt this entity linker to map $h, t$ to $h_k, t_k$.
%     \item Relation mapping. We largely follow the relation mapping method proposed by \cite{angeli2015leveraging} to construct an offline relation map between KG predicates and relation phrases of triples. The basic idea is that the more often the entity pairs of the triples and KG facts are linked, the more likely the corresponding relations are mapped to each other. In addition, we normalize each relation phrase of the triples by lemmatization, and removing inflection, auxiliary verbs, adjectives, adverbs. After the relation mapping is constructed, one author manually checks whether the top 15 relation phrases are true mappings for each KG predicate. We only reserve the true ones in the final relation mapping. This process takes approximately one day. At test time, $r$ is mapped to $r_k$ with a look-up operation in the relation mapping.
% \end{itemize}
% Additional details of the map function are described in Appendix~\ref{sec:implement}.

% In addition, like with previous OIE systems, we want a way to trade recall for precision by tuning a confidence threshold. We directly use the total attention score associated with each triple as the threshold, and tune it on a hold-out dataset. 


    % The document collection mainly consists of newswire data. Besides, entities with well-populated KG entries (either in the official TAC KBP KG or in online resources such as Wikipedia) are generally avoided as query entities. Therefore we experimented with the official TAC KBP KG in the 2013 challenge as the  KG. This dataset serves the  evaluation for both BERT and GPT-2.
    
    
% We compare with the following OIE systems. (\expandafter{\romannumeral1}) Neural network (NN) based OIE:
% SenseOIE~\cite{roy2019supervising}, 
% SpanOIE~\cite{zhan2020span}\footnote{\tiny\url{https://github.com/zhanjunlang/Span_OIE}},
% RnnOIE~\cite{stanovsky2018supervised}\footnote{\tiny\url{https://github.com/gabrielStanovsky/supervised-oie}},
% NeuralOIE~\cite{cui2018neural}\footnote{\tiny We use the BERT implementation (CopyAttn+BERT) available at \url{https://github.com/dair-iitd/imojie}},
% IMoJIE~\cite{kolluru2020imojie}\footnote{\tiny\url{https://github.com/dair-iitd/imojie}},
% Multi$^2$OIE~\cite{ro2020multi}\footnote{\tiny\url{https://github.com/youngbin-ro/Multi2OIE}},
% and OpenIE6~\cite{kolluru2020openie6}\footnote{\tiny\url{https://github.com/dair-iitd/openie6}}.
% (\expandafter{\romannumeral2}) Linguistic pattern based OIE:  MinIE~\cite{gashteovski2017minie}\footnote{\tiny\url{https://github.com/uma-pi1/minie}}, ClausIE~\cite{del2013clausie}\footnote{\tiny\url{https://www.mpi-inf.mpg.de/departments/databases-and-information-systems/research/ambiverse-nlu/clausie}}, OLLIE~\cite{schmitz2012open}\footnote{\tiny\url{https://github.com/knowitall/ollie}}, PropS~\cite{stanovsky2016getting}\footnote{\tiny\url{https://github.com/gabrielStanovsky/props}}, OpenIE4~\cite{christensen2011analysis}\footnote{\tiny\url{https://github.com/allenai/openie-standalone}}, OpenIE5~\cite{saha2017bootstrapping,saha2018open}\footnote{\label{ft:openie51}\tiny\url{https://github.com/dair-iitd/OpenIE-standalone}}, and Stanford OpenIE~\cite{angeli2015leveraging}.
% Note that all the NN OIE systems are supervised.

% IMoJIE~\cite{kolluru2020imojie}\footnote{\tiny\url{https://github.com/dair-iitd/imojie}} is a sequence generation OIE model that uses BERT at encoding time.
%     \item Multi$^2$OIE~\cite{ro2020multi}\footnote{\tiny\url{https://github.com/youngbin-ro/Multi2OIE}} models OIE as a sequence-labeling problem that combines BERT with multi-head attention blocks.
%     \item OpenIE6~\cite{kolluru2020openie6}\footnote{\tiny\url{https://github.com/dair-iitd/openie6}} is one of the state-of-the-art OIE systems. It treats OIE as a 2-D grid labeling task, and trains a BERT like architecture for the task.


% To verify the ability to produce correct relational knowledge, we compare the extractions of pre-trained LMs to the outputs of two open information extraction (OIE) systems below, which also produce triples in the form of $(h, r, t)$.


% We find that relational knowledge in pre-trained LMs generalizes well to out-of-domain scenarios. We particularly find that all our methods achieve competitive precision, which is greater than 60\%. Specifically, they outperform the linguistic-based OIE systems. We anticipate this is because the patterns captured in parameters (i.e., attention weights) are more flexible to capture unseen entities and relations compared to the fixed manually created linguistic patterns in OpenIE 5.1 and Stanford OpenIE. Similar to the observations on the in-domain dataset, we find that the knowledge calibration is both effective and efficient. Even though all pre-trained LMs outperform the OIE systems in the recall, improving recall is clearly the future direction. We find that the main cause of the moderate recall is the incorrect entities caused by spaCy noun chunks as summarized in Sec.~\ref{sec:error}.
% % capture unseen entities and relations compared to the fixed manually created linguistic patterns in OpenIE 5.1 and Stanford OpenIE.
% % Compared to supervised model-based OIE system OpenIE 6, the pre-trained attention weights have captured a wider set of knowledgeable patterns. 
% % they outperform both linguistic-based and neural network-based OIE

% % \input{tabs/resulttac}

% We also find that the out-of-domain performance is comparable with the in-domain performance. But we do see that BERT$_{\rm LARGE}$ outperforms Stanford OpenIE by approximately 1.98\% in F1. The F1 gain is smaller compared to that on in-domain Wikidata. This shows that the in-domain knowledge is easier to be collected compared to the out-of-domain knowledge. Overall, this shows that pre-trained LMs have captured both out-of-domain and in-domain general knowledge. 

% Similar to the observations on in-domain Wikidata, larger or deeper LMs also store richer out-of-domain relational knowledge. BERT$_{\rm LARGE}$ outperforms BERT$_{\rm BASE}$ since the doubling parameter size. GPT-2s share similar trends, where we observe performance increases when the model size increases. Moreover, we find that BERT LMs outperform GPT-2 LMs under similar model sizes. In particular, BERT$_{\rm BASE}$ performs better than GPT-2 in F1, and BERT$_{\rm LARGE}$ outperforms GPT-2$_{\rm MEDIUM}$ in F1. BERT$_{\rm BASE}$ and GPT-2 are similar in size, while BERT$_{\rm LARGE}$ and GPT-2$_{\rm MEDIUM}$ are similar in model size. This is mainly because the recall of BERT LMs is higher than that of corresponding GPT-2 LMs. The result indicates that the Cloze-style loss function (i.e., masked language model) of BERT is more effective and flexible in recovering more knowledge than the autoregressive LM objective. We also notice that the precision of GPT-2 LMs is higher than that of BERT LMs. The reason is that the autoregressive LM objective captures more accurate knowledge than Cloze-style loss does by not introducing extra noise (e.g., masked tokens) during pre-training.



% Table~\ref{tab:resultwiki} summarizes the results on the in-domain benchmark, Wikidata. We find that pre-trained LMs in particular BERT LMs contain improved in-domain relational knowledge compared to OIE systems. The results suggest that pre-training on in-domain corpus is effective in integrating general relational knowledge into the parameters of the LMs. This is also encouraging since pre-training is shown at least comparable in recalling knowledge with linguistic-based OIE systems. Both OpenIE 5.1 and Stanford OpenIE are derived from manually designed linguistic patterns based on dependency parsing or POS tag. 
% % The state-of-the-art OpenIE 6 trains a BERT like architecture for the extraction task.
% This shows that the pre-trained attention weights capture more flexible and a wider set of patterns in terms of knowledgeable information in a sentence. In addition to the conclusion in LAMA~\cite{petroni2019language}, we demonstrate that general in-domain knowledge without relation specification is available in pre-trained LMs. We also find that BERT$_{\rm LARGE}$ outperforms BERT$_{\rm BASE}$. This shows that the larger model (BERT$_{\rm LARGE}$ has approximately 3x more parameters compared to BERT$_{\rm BASE}$) contains more in-domain knowledge. When larger or deeper models that include Wikipedia in the pre-training data are tested on our in-domain benchmark, we can expect more gains compared to the OIE systems. Besides, the precision is higher compared to recall. Wikidata is not fully built from Wikipedia, we could improve the recall by running on larger corpora such as WebText2 and Common Crawl~\citep{abs-1910-10683,brown2020language} to collect more triples.
% % \input{tabs/resultwiki}
% \input{tabs/resultall}
% \input{tabs/runtime}

% % 
% %  or supervised model-based OIE systems

% We also show that the knowledge calibration module in Sec.~\ref{sec:app} is both effective in extracting relational knowledge and efficient for large-scale quantitative evaluation. We obtain better precision, recall, and F1 scores compared to OIE systems. This means the knowledge calibration is capable of recovering the knowledge. We argue that this means we are measuring a lower bound for what LMs have. For example, we can also incorporate relations that are not between the entity pairs as we observe a number of facts are in inverted sentences. We leave this as one of future explorations. For the efficiency benefits, the main reason is that beam search is efficient in exploring the relational sequences in the input sentence. Besides, the attention scores used in the beam search are produced via a single forward pass of the pre-trained LM over the input sentence without fine-tuning, which is also computationally efficient. The results suggest that our evaluation framework is scalable to larger benchmarks. 


% % \subsection{Out-of-Domain Results}

% % \subsubsection{TAC KBP-OIE}


% \paragraph{Problem Definition} We assume the relational knowledge in a pre-trained LM is in a triple format {\sl (head, relation, tail)}~\footnote{\tiny{We use the term ``head'' and ``tail'' to denote head and tail's ``entities'' or ``entity mentions'' for simplicity.}}, in short, $(h, r, t)$. We approach the following problem: Given a textual corpus and a pre-trained LM, a set of triples \{$(h, r, t)$\} is extracted from the corpus using the parameters of the LM, and returned representing the relational knowledge in the pre-trained LM. For example, in Figure~\ref{fig:overview}, \{{\sl (Dylan, is, songwriter)}, {\sl (Dylan, awarded, Nobel Prize)}\} is returned. We use the same formalization for both in-domain and out-of-domain evaluation.
% {\sl (head, relation, tail)}, in short, $(h, r, t)$

% \subsection{Argument Extraction}

% We treat every

% The search takes a noun phrase (NP) chunked sentence from the corpus as input. 
% The attention scores are from the forward pass of the LM over the sentence. 
% We consider a pair of NP chunks as an entity pair. 

 conditioned on their type signatures matching
 
 with an unsupervised entity linker based on an unsupervised mention-to-entity dictionary~\citep{spitkovsky2012cross}, which is
 
 \input{tabs/entity_linking_human_eval}

\input{tabs/entity_linking_gold}

We additional conduct human evaluation over 5 sampled Wikipedia articles (see Table~\ref{tab:el_human_eval}) and evaluation against gold mentions in 100 sampled Wikipedia articles (see Table~\ref{tab:el_gold}), and the results show that our unsupervised entity linker achieves a precision about 67.4\% and a recall on gold mentions about 76.71\%.


(\expandafter{\romannumeral1}) Neural OIE systems:
SenseOIE~\citep{roy2019supervising}, 
SpanOIE~\citep{zhan2020span},
RnnOIE~\citep{stanovsky2018supervised},
NeuralOIE~\citep{cui2018neural},
IMoJIE~\citep{kolluru2020imojie},
Multi$^2$OIE~\citep{ro2020multi},
and OpenIE6~\citep{kolluru2020openie6}.
(\expandafter{\romannumeral2}) Linguistic OIE systems: MinIE~\citep{gashteovski2017minie}, ClausIE~\citep{del2013clausie}, OLLIE~\citep{schmitz2012open}, PropS~\citep{stanovsky2016getting}, OpenIE4~\citep{christensen2011analysis}, OpenIE5~\citep{saha2017bootstrapping,saha2018open}, and Stanford OpenIE~\citep{angeli2015leveraging}.

BERT$_{\rm BASE}$ and GPT-2 are similar in size, while BERT$_{\rm LARGE}$ and GPT-2$_{\rm MEDIUM}$ are similar in model size. 

% \tiny{There are 2,383 correct gold triples based on the ``manual runs'' assessment.}}.
% \footnoteref{ft:anydoc}  
% ~\footnote{\label{ft:anydoc}



%Recently, automated prompts~\citep{wallace-etal-2019-universal,shin2020autoprompt,li2021prefix,liu2021gpt} are created to cause the corresponding LMs to produce desired knowledge. 
%including WebQuestion~\citep{berant2013semantic}, NaturalQuestion~\citep{kwiatkowski2019natural} and TriviaQA~\citep{joshi2017triviaqa} 
%, which considers the general relational information in pre-trained LMs instead of specific relations. 
%Studies have leveraged the pre-trained LMs as virtual knowledge graphs (KG), and show reasonable performance in QA tasks~\citep{dhingra2020differentiable,guu2020realm}, and language modeling~\citep{khandelwal2019generalization}. LMs are further enhanced by KGs~\citep{peters2019knowledge} to improve the performance on knowledge-driven benchmarks. 
%Our benchmark is generally relevant to the KG construction work, which can be generally categorized into two groups, (\expandafter{\romannumeral1}) supervised approaches, and (\expandafter{\romannumeral2}) semi-supervised approaches. Supervised KGs include Wikidata, Freebase~\citep{bollacker2008freebase}, YAGO~\citep{suchanek2007yago}, YAGO2~\citep{hoffart2013yago2}, DBpedia~\citep{auer2007dbpedia}, which are built based on human contribution from Wikipedia infoboxes and other structured data sources.

==> tabs/entity_linking_gold.tex <==
\begin{table}[t]
\small
\renewcommand\tabcolsep{4.5pt}
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Recall} & \textbf{\begin{tabular}[c]{@{}l@{}}Gold mentions\\ in prediction\end{tabular}} & \textbf{F1} & \textbf{\begin{tabular}[c]{@{}l@{}}\# of gold \\ mention\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\# of \\ preidction\end{tabular}} \\ \midrule
76.71\%         & 24.85\%                                                                        & 37.54\%     & 1035                                                                   & 3195                                                                 \\ \bottomrule
\end{tabular}
\caption{Evaluation against gold mentions in 100 sampled Wikipedia articles. Noted that the gold mentions in Wikipedia is highly incomplete.}
\label{tab:el_gold}
\end{table}

==> tabs/entity_linking_human_eval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\small
\renewcommand\tabcolsep{5.5pt}
\begin{tabular}{@{}clllc@{}}
\toprule
\multicolumn{4}{c}{\textbf{Annotation}}                                                                                                            & \multirow{2}{*}{\textbf{Total}} \\ \cmidrule(r){1-4}
\textbf{Correct}                & \multicolumn{1}{c}{\textbf{Wrong}} & \multicolumn{1}{c}{\textbf{Overfit}} & \multicolumn{1}{c}{\textbf{Missing}} &                                 \\ \midrule
\multicolumn{1}{l}{91 (67.4\%)} & 15 (11.1\%)                        & 27 (20.0\%)                          & 2 (1.5\%)                            & \multicolumn{1}{l}{135}         \\ \bottomrule
\end{tabular}
\caption{Human evaluation for entity linker on 135 entity mentions over 5 sampled Wikipedia articles.}
\label{tab:el_human_eval}
\end{table}

==> tabs/resultallbak.tex <==
% \begin{table*}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ll|llll|llll|llll|llll}
% \toprule
% \multirow{2}{*}{{\bf Method}} & \multirow{2}{*}{{\bf \#Params}} & \multicolumn{4}{c|}{{\bf CaRB}}  & \multicolumn{4}{c|}{{\bf Re-OIE2016}} & \multicolumn{4}{c|}{\bf{TAC KBP-OIE}} & \multicolumn{4}{c}{\bf{Wikidata-OIE}}   \\
%                         &                           & P    & R    & F1   & AUC  & P      & R     & F1    & AUC   & P     & R     & F1    & AUC & P      & R      & F1     & AUC \\
% \midrule
% MinIE                   & -                         & -    & -    & 41.9 & -    & 48.22      & 71.1     & 57.5     & 47.2     &  -     &  -     & -      & -    &  -      &  -      & -       & -    \\
% ClausIE                 & -                         & -    & -    & 44.9 & 22.4 & -      & -     & 64.2  & 46.4  &   -    &   -    &  -     &  -   &   -     &  -      & -       &  -   \\
% OLLIE                   & -                         & -    & -    & 41.1 & 22.4 & -      & -     & 49.5  & 31.3  &  -     &   -    &  -     &   -  &   -     &  -      &  -      &  -   \\
% PropS                   & -                         & -    & -    & 31.9 & 12.6 & -      & -     & 64.2  & 43.3  &  -     & -      &  -     & -    &   -     &  -      &  -      &  -   \\
% OpenIE 4                & -                         & -    & -    & 48.8 & 27.2 & -      & -     & 68.3  & 50.9  & 52.86     & 14.18     & 22.36     & -   & 30.62  & 13.98  & 19.20 & -   \\
% OpenIE 5                & -                         & -    & -    & 48.0 & 25.0 & 61.1      & 76.5     & 67.9     & 45.8     & 56.98 & 14.54 & 23.16 & -   & 26.26 & 14.38 & 18.58 & -   \\
% Stanford OpenIE         & -                         & -    & -    & 23.0 & 13.4 & -      & -     & 16.7  & 11.5  & 61.55 & 17.35 & 27.07 & -   & 23.32  & 13.09  & 16.77  & -   \\
%  \hdashline
% SenseOIE                & 640K                         & -    & -    & 28.2 & -    & -      & -     & -     & -     &       &       &       &     &        &        &        &     \\
% SpanOIE                 & 963K                         & 60.9 & 41.6 & 49.4 & 30.0 & 79.7   & 74.5  & 77.0  & 65.8  &       &       &       &     &        &        &        &     \\
% RnnOIE                  & 965K                         & 55.6 & 40.2 & 46.7 & 26.8 & 84.2   & 73.9  & 78.7  & 68.3  &  50.00    &  14.56  & 22.55  & -  & 29.88  & 15.87  & 20.73  & -   \\
% NeuralOIE               & 5M                         & -    & -    & 51.6 & 32.8 & 79.2      & 77.5     & 78.4     & 73.0     &       &       &       &     &        &        &        &     \\
% IMOJIE                  & 110M                         & 64.7    & 45.6    & 53.5 & 33.3 & 88.1   & 67.1  & 76.2  & 63.1  &    58.21   &   14.94    &    23.78   &   -  &     31.22   &   16.19     &    21.32    &  -   \\
% Multi$^2$OIE               &       110M                  & 60.9 & 45.8 & 52.3 & 32.6 & 86.9   & 81.0  & 83.9  & 74.6  &     -  & -      &    -   &    - &    -    &    -    &     -   &   -  \\
% OpenIE 6                & 220M                         & -    & -    & 54.0 & 35.7 & 75.3      & 78.2     & 76.7     & 73.8     & 60.00 & 14.94 & 23.92     & -   & 29.84 & 15.34 & 20.26 & -   \\
%  \hdashline
% BERT$_{\rm BASE}$ \ours            & 109M                      & 21.2 & 18.3 & 19.7 & - & 25.9 & 34.0 & 29.4 & - & 61.57 & 18.79 & 28.79 & -   & 31.99 & 18.85 & 23.72 & -   \\
% BERT$_{\rm LARGE}$  \ours           & 335M                      & 22.4 & 20.2 & 21.2 & - & 30.7 & 38.5 & 34.1 & - & 61.69 & 18.99 & 29.05 & -   & 32.25  & 19.10  & 23.99  & -   \\
% GPT-2   \ours                & 117M                      & 23.1 & 19.8 & 21.3 & - & 25.1 & 38.3 & 30.3 & - & 61.62 & 18.17 & 28.07 & -   & 32.37      & 18.08      & 23.20      & -   \\
% GPT-2$_{\rm MEDIUM}$  \ours         & 345M                      & 23.7 & 20.0 & 21.7 & - & 26.8 & 39.9 & 32.0 & - & 62.10 & 18.65 & 28.69 & -   & 33.12      & 18.10      & 23.41      & -   \\
% GPT-2$_{\rm LARGE}$  \ours          & 774M                      & 24.2 & 20.5 & 22.2 & - & 27.4 & 41.6 & 33.0 & - & \secbest 62.38 & \secbest 19.00 & \secbest 29.12 & -   & \secbest 34.23      & \secbest 18.11      & \secbest 23.69      & -   \\
% GPT-2$_{\rm XL}$  \ours             & 1558M                     & 24.5 & 21.0 & 22.7 & - & 29.3 & 43.4 & 35.0 & - & \best 62.69 & \best  19.47 & \best 29.72 & -   & \best 35.74      & \best 18.51      & \best 24.39      & -  \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Compare the quality of different OIE systems.\xiao{update ?}\todo{add ours, best hightlight, supervised method marker}}
% \label{tab:resultall}
% \end{table*}


\comm{
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllllllllllll}
\multirow{2}{*}{Method} & \multirow{2}{*}{\#Params} & \multicolumn{4}{l}{CaRB}  & \multicolumn{4}{l}{Re-OIE2016} & \multicolumn{4}{l}{TAC KBP} & \multicolumn{4}{l}{Wikidata}   \\
                        &                           & P    & R    & F1   & AUC  & P      & R     & F1    & AUC   & P     & R     & F1    & AUC & P      & R      & F1     & AUC \\
MinIE                   & -                         & -    & -    & 41.9 & -    &        &       &       &       &       &       &       &     &        &        &        &     \\
ClausIE                 & -                         & -    & -    & 44.9 & 22.4 & -      & -     & 64.2  & 46.4  &       &       &       &     &        &        &        &     \\
OLLIE                   & -                         & -    & -    & 41.1 & 22.4 & -      & -     & 49.5  & 31.3  &       &       &       &     &        &        &        &     \\
PropS                   & -                         & -    & -    & 31.9 & 12.6 & -      & -     & 64.2  & 43.3  &       &       &       &     &        &        &        &     \\
OpenIE 4                & -                         & -    & -    & 48.8 & 27.2 & -      & -     & 68.3  & 50.9  &       &       &       &     &        &        &        &     \\
OpenIE 5                & -                         & -    & -    & 48.0 & 25.0 &        &       &       &       & 56.98 & 14.54 & 23.16 & ?   & 26.26? & 14.38? & 18.58? & ?   \\
Stanford OpenIE         & -                         & -    & -    & 23.0 & 13.4 & -      & -     & 16.7  & 11.5  & 61.55 & 17.35 & 27.07 & ?   & 23.32  & 13.09  & 16.77  & ?   \\
SenseOIE                & ?                         & -    & -    & 28.2 & -    &        &       &       &       &       &       &       &     &        &        &        &     \\
SpanOIE                 & ?                         & 60.9 & 41.6 & 49.4 & 30.0 & 79.7   & 74.5  & 77.0  & 65.8  &       &       &       &     &        &        &        &     \\
RnnOIE                  & ?                         & 55.6 & 40.2 & 46.7 & 26.8 & 84.2   & 73.9  & 78.7  & 68.3  & ?     & ?     & ?     & ?   & 28.51  & 14.65  & 19.36  & ?   \\
NeuralOIE               & ?                         & -    & -    & 51.6 & 32.8 &        &       &       &       &       &       &       &     &        &        &        &     \\
IMOJIE                  & ?                         & -    & -    & 53.5 & 33.3 &        &       &       &       &       &       &       &     &        &        &        &     \\
Multi2OIE               & ?                         & 60.9 & 45.8 & 52.3 & 32.6 & 86.9   & 81.0  & 83.9  & 74.6  &       &       &       &     &        &        &        &     \\
OpenIE 6                & ?                         & -    & -    & 52.7 & 33.7 &        &       &       &       & ?     & ?     & ?     & ?   & ?      & ?      & ?      & ?   \\
BERT\_base              & 109M                      & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 61.57 & 18.79 & 28.79 & ?   & 32.29? & 13.78? & 19.32? & ?   \\
BERT\_large             & 335M                      & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 61.69 & 18.99 & 29.05 & ?   & 29.08  & 18.61  & 22.70  & ?   \\
GPT-2                   & 117M                      & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 61.62 & 18.17 & 28.07 & ?   & ?      & ?      & ?      & ?   \\
GPT-2\_medium           & 345M                      & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 62.10 & 18.65 & 28.69 & ?   & ?      & ?      & ?      & ?   \\
GPT-2\_large            & 774M                      & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 62.38 & 19.00 & 29.12 & ?   & ?      & ?      & ?      & ?   \\
GPT-2\_xl               & 1558M                     & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 62.69 & 19.47 & 29.72 & ?   & ?      & ?      & ?      & ?  \\
\end{tabular}%
}
\caption{}
\label{tab:my-table}
\end{table}
}


\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|cccc|cccc|ccc|ccc}
\toprule
\multirow{2}{*}{{\bf Method}} & \multirow{2}{*}{{\bf \#Params}} & \multicolumn{4}{c|}{{\bf CaRB}}  & \multicolumn{4}{c|}{{\bf Re-OIE2016}} & \multicolumn{3}{c|}{\bf{TAC KBP-OIE}} & \multicolumn{3}{c}{\bf{Wikidata-OIE}}   \\
                        &                           & P    & R    & F1   & AUC  & P      & R     & F1    & AUC   & P     & R     & F1     & P      & R      & F1     \\
\midrule
MinIE~\citep{gashteovski2017minie}                   & -                         & -    & -    & 41.9 & -    & 48.2      & 71.1     & 57.5     & 47.2     &  -     &  -     & -      &  -      &  -      & -          \\
ClausIE~\citep{del2013clausie}                 & -                         & -    & -    & 44.9 & 22.4 & -      & -     & 64.2  & 46.4  &   -    &   -    &  -     &  -   &   -     &  -      \\
OLLIE~\citep{schmitz2012open}                   & -                         & -    & -    & 41.1 & 22.4 & -      & -     & 49.5  & 31.3  &  -     &   -    &  -     &   -  &   -     &  -      \\
PropS~\citep{stanovsky2016getting}                   & -                         & -    & -    & 31.9 & 12.6 & -      & -     & 64.2  & 43.3  &  -     & -      &  -     & -    &   -     &  -     \\
OpenIE4~\citep{christensen2011analysis}                & -                         & -    & -    & 48.8 & 27.2 & -      & -     & 68.3  & 50.9  & 52.9     & 14.2     & 22.4        & 30.6  & 14.0  & 19.2    \\
OpenIE5~\citep{saha2017bootstrapping,saha2018open}                & -                         & -    & -    & 48.0 & 25.0 & 61.1      & 76.5     & 67.9     & 45.8     & 57.0 & 14.6 & 23.2   & 26.3 & 14.4 & 18.6   \\
Stanford OpenIE$^*$~\citep{angeli2015leveraging}         & -                         & -    & -    & 23.0 & 13.4 & -      & -     & 16.7  & 11.5  & 61.6 & 17.4 & 27.1 & 23.3  & 13.1  & 16.8    \\
 \hdashline
SenseOIE$^*$~\citep{roy2019supervising}                & 640K                         & -    & -    & 28.2 & -    & -      & -     & -     & -     &  -     &    -   &   -    &  -   &   -     &     -    \\
SpanOIE$^*$~\citep{zhan2020span}                 & 963K                         &  60.9 & 41.6 & 49.4 & 30.0 & 79.7   & 74.5  & 77.0  & 65.8  &   -    &     -  &     -  &  -   &     -   &      -   \\
NeuralOIE$^*$~\citep{cui2018neural}               & 5M                         & -    & -    & 51.6 & 32.8 & 79.2      & 77.5     & 78.4     & 73.0     &   -    &     -  &     -  &   -  &    -    &    -    \\
Multi$^2$OIE$^*$~\citep{ro2020multi}               &       110M                  &  60.9 & \best 45.8 & 52.3 & 32.6 &  86.9   & \best 81.0  & \best 83.9  & \best 74.6  &     -  & -      &    -   &    - &    -    &    -    \\
RnnOIE$^*$~\citep{stanovsky2018supervised}                  & 965K                         & 55.6 & 40.2 & 46.7 & 26.8 & 84.2   & 73.9  &  78.7  & 68.3  &  50.0    &  14.6  & 22.6  & 29.9  & 15.9  & 20.7    \\
IMOJIE$^*$~\citep{kolluru2020imojie}                  & 110M                         & \best 64.7    &  45.6    &  53.5 &  33.3 & \best 88.1   & 67.1  & 76.2  & 63.1  &    58.2   &   14.9    &    23.8     &     31.2   &   16.2     &    21.3     \\
OpenIE6$^*$~\citep{kolluru2020openie6}                & 220M                         & -    & -    & \best 54.0 & \best 35.7 & 75.3      &  78.2     & 76.7     &  73.8     & 60.0 & 14.9 & 23.9      & 29.8 & 15.3 & 20.3   \\
 \hdashline
BERT$_{\rm BASE}$ (zero-shot) \ours            & 109M                      & 21.2 & 18.3 & 19.7 & - & 25.9 & 34.0 & 29.4 & - & 61.6 & 18.8 & 28.8    & 32.0 &  18.9 & 23.7   \\
BERT$_{\rm LARGE}$ (zero-shot) \ours           & 335M                      & 22.4 & 20.2 & 21.2 & - & 30.7 & 38.5 & 34.1 & - & 61.7 & 19.0 & 29.1   & 32.3  & \best 19.1  &  24.0    \\
GPT-2 (zero-shot)  \ours                & 117M                      & 23.1 & 19.8 & 21.3 & - & 25.1 & 38.3 & 30.3 & - & 61.6 & 18.2 & 28.1   & 32.4      & 18.1      & 23.2       \\
GPT-2$_{\rm MEDIUM}$ (zero-shot) \ours         & 345M                      & 23.7 & 20.0 & 21.7 & - & 26.8 & 39.9 & 32.0 & - & 62.1 & 18.7 & 28.7    & 33.1      & 18.2      & 23.5       \\
GPT-2$_{\rm LARGE}$ (zero-shot) \ours          & 774M                      & 24.2 & 20.5 & 22.2 & - & 27.4 & 41.6 & 33.0 & - &  62.4 &  19.0 &  29.1   &  34.2      & 18.3      & 23.8        \\
GPT-2$_{\rm XL}$ (zero-shot) \ours             & 1558M                     & 24.5 & 21.0 & 22.7 & - & 29.3 & 43.4 & 35.0 & - & \best 62.7 & \best  19.5 & \best 29.7   & \best 35.7      & 18.5      & \best 24.4      \\
\bottomrule
\end{tabular}%
}
\caption{Compare the quality of different OIE systems. An asterisk (*) indicates a supervised method. \xiao{update ?}\todo{add ours, best hightlight, supervised method marker}}
\label{tab:resultall}
\end{table*}

\comm{
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|cccc|cccc|cccc|cccc}
\toprule
\multirow{2}{*}{{\bf Method}} & \multirow{2}{*}{{\bf \#Params}} & \multicolumn{4}{c|}{{\bf CaRB}}  & \multicolumn{4}{c|}{{\bf Re-OIE2016}} & \multicolumn{4}{c|}{\bf{TAC KBP-OIE}} & \multicolumn{4}{c}{\bf{Wikidata-OIE}}   \\
                        &                           & P    & R    & F1   & AUC  & P      & R     & F1    & AUC   & P     & R     & F1    & AUC & P      & R      & F1     & AUC \\
\midrule
MinIE~\citep{gashteovski2017minie}                   & -                         & -    & -    & 41.9 & -    & 48.2      & 71.1     & 57.5     & 47.2     &  -     &  -     & -      & -    &  -      &  -      & -       & -    \\
ClausIE~\citep{del2013clausie}                 & -                         & -    & -    & 44.9 & 22.4 & -      & -     & 64.2  & 46.4  &   -    &   -    &  -     &  -   &   -     &  -      & -       &  -   \\
OLLIE~\citep{schmitz2012open}                   & -                         & -    & -    & 41.1 & 22.4 & -      & -     & 49.5  & 31.3  &  -     &   -    &  -     &   -  &   -     &  -      &  -      &  -   \\
PropS~\citep{stanovsky2016getting}                   & -                         & -    & -    & 31.9 & 12.6 & -      & -     & 64.2  & 43.3  &  -     & -      &  -     & -    &   -     &  -      &  -      &  -   \\
OpenIE4~\citep{christensen2011analysis}                & -                         & -    & -    & 48.8 & 27.2 & -      & -     & 68.3  & 50.9  & 52.9     & 14.2     & 22.4     & -   & 30.6  & 14.0  & 19.2 & -   \\
OpenIE5~\citep{saha2017bootstrapping,saha2018open}                & -                         & -    & -    & 48.0 & 25.0 & 61.1      & 76.5     & 67.9     & 45.8     & 57.0 & 14.6 & 23.2 & -   & 26.3 & 14.4 & 18.6 & -   \\
Stanford OpenIE$^*$~\citep{angeli2015leveraging}         & -                         & -    & -    & 23.0 & 13.4 & -      & -     & 16.7  & 11.5  & 61.6 & 17.4 & 27.1 & -   & 23.3  & 13.1  & 16.8  & -   \\
 \hdashline
SenseOIE$^*$~\citep{roy2019supervising}                & 640K                         & -    & -    & 28.2 & -    & -      & -     & -     & -     &  -     &    -   &   -    &  -   &   -     &     -   &   -     &  -   \\
SpanOIE$^*$~\citep{zhan2020span}                 & 963K                         &  60.9 & 41.6 & 49.4 & 30.0 & 79.7   & 74.5  & 77.0  & 65.8  &   -    &     -  &     -  &  -   &     -   &      -  &  -      &   -  \\
NeuralOIE$^*$~\citep{cui2018neural}               & 5M                         & -    & -    & 51.6 & 32.8 & 79.2      & 77.5     & 78.4     & 73.0     &   -    &     -  &     -  &   -  &    -    &    -    &  -      &  -   \\
Multi$^2$OIE$^*$~\citep{ro2020multi}               &       110M                  &  60.9 & \best 45.8 & 52.3 & 32.6 &  86.9   & \best 81.0  & \best 83.9  & \best 74.6  &     -  & -      &    -   &    - &    -    &    -    &     -   &   -  \\
RnnOIE$^*$~\citep{stanovsky2018supervised}                  & 965K                         & 55.6 & 40.2 & 46.7 & 26.8 & 84.2   & 73.9  &  78.7  & 68.3  &  50.0    &  14.6  & 22.6  & -  & 29.9  & 15.9  & 20.7  & -   \\
IMOJIE$^*$~\citep{kolluru2020imojie}                  & 110M                         & \best 64.7    &  45.6    &  53.5 &  33.3 & \best 88.1   & 67.1  & 76.2  & 63.1  &    58.2   &   14.9    &    23.8   &   -  &     31.2   &   16.2     &    21.3    &  -   \\
OpenIE6$^*$~\citep{kolluru2020openie6}                & 220M                         & -    & -    & \best 54.0 & \best 35.7 & 75.3      &  78.2     & 76.7     &  73.8     & 60.0 & 14.9 & 23.9     & -   & 29.8 & 15.3 & 20.3 & -   \\
 \hdashline
BERT$_{\rm BASE}$ (zero-shot) \ours            & 109M                      & 21.2 & 18.3 & 19.7 & - & 25.9 & 34.0 & 29.4 & - & 61.6 & 18.8 & 28.8 & -   & 32.0 &  18.9 & 23.7 & -   \\
BERT$_{\rm LARGE}$ (zero-shot) \ours           & 335M                      & 22.4 & 20.2 & 21.2 & - & 30.7 & 38.5 & 34.1 & - & 61.7 & 19.0 & 29.1 & -   & 32.3  & \best 19.1  &  24.0  & -   \\
GPT-2 (zero-shot)  \ours                & 117M                      & 23.1 & 19.8 & 21.3 & - & 25.1 & 38.3 & 30.3 & - & 61.6 & 18.2 & 28.1 & -   & 32.4      & 18.1      & 23.2      & -   \\
GPT-2$_{\rm MEDIUM}$ (zero-shot) \ours         & 345M                      & 23.7 & 20.0 & 21.7 & - & 26.8 & 39.9 & 32.0 & - & 62.1 & 18.7 & 28.7 & -   & 33.1      & 18.2      & 23.5      & -   \\
GPT-2$_{\rm LARGE}$ (zero-shot) \ours          & 774M                      & 24.2 & 20.5 & 22.2 & - & 27.4 & 41.6 & 33.0 & - &  62.4 &  19.0 &  29.1 & -   &  34.2      & 18.3      & 23.8      & -   \\
GPT-2$_{\rm XL}$ (zero-shot) \ours             & 1558M                     & 24.5 & 21.0 & 22.7 & - & 29.3 & 43.4 & 35.0 & - & \best 62.7 & \best  19.5 & \best 29.7 & -   & \best 35.7      & 18.5      & \best 24.4      & -  \\
\bottomrule
\end{tabular}%
}
\caption{Compare the quality of different OIE systems. An asterisk (*) indicates a supervised method. \xiao{update ?}\todo{add ours, best hightlight, supervised method marker}}
\label{tab:resultall}
\end{table*}

\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllllllllllll}
\multirow{2}{*}{Method} & \multirow{2}{*}{\#Params} & \multicolumn{4}{l}{CaRB}  & \multicolumn{4}{l}{Re-OIE2016} & \multicolumn{4}{l}{TAC KBP} & \multicolumn{4}{l}{Wikidata}   \\
                        &                           & P    & R    & F1   & AUC  & P      & R     & F1    & AUC   & P     & R     & F1    & AUC & P      & R      & F1     & AUC \\
MinIE                   & -                         & -    & -    & 41.9 & -    &        &       &       &       &       &       &       &     &        &        &        &     \\
ClausIE                 & -                         & -    & -    & 44.9 & 22.4 & -      & -     & 64.2  & 46.4  &       &       &       &     &        &        &        &     \\
OLLIE                   & -                         & -    & -    & 41.1 & 22.4 & -      & -     & 49.5  & 31.3  &       &       &       &     &        &        &        &     \\
PropS                   & -                         & -    & -    & 31.9 & 12.6 & -      & -     & 64.2  & 43.3  &       &       &       &     &        &        &        &     \\
OpenIE 4                & -                         & -    & -    & 48.8 & 27.2 & -      & -     & 68.3  & 50.9  &       &       &       &     &        &        &        &     \\
OpenIE 5                & -                         & -    & -    & 48.0 & 25.0 &        &       &       &       & 56.98 & 14.54 & 23.16 & ?   & 26.26? & 14.38? & 18.58? & ?   \\
Stanford OpenIE         & -                         & -    & -    & 23.0 & 13.4 & -      & -     & 16.7  & 11.5  & 61.55 & 17.35 & 27.07 & ?   & 23.32  & 13.09  & 16.77  & ?   \\
SenseOIE                & ?                         & -    & -    & 28.2 & -    &        &       &       &       &       &       &       &     &        &        &        &     \\
SpanOIE                 & ?                         & 60.9 & 41.6 & 49.4 & 30.0 & 79.7   & 74.5  & 77.0  & 65.8  &       &       &       &     &        &        &        &     \\
RnnOIE                  & ?                         & 55.6 & 40.2 & 46.7 & 26.8 & 84.2   & 73.9  & 78.7  & 68.3  & ?     & ?     & ?     & ?   & 28.51  & 14.65  & 19.36  & ?   \\
NeuralOIE               & ?                         & -    & -    & 51.6 & 32.8 &        &       &       &       &       &       &       &     &        &        &        &     \\
IMOJIE                  & ?                         & -    & -    & 53.5 & 33.3 &        &       &       &       &       &       &       &     &        &        &        &     \\
Multi2OIE               & ?                         & 60.9 & 45.8 & 52.3 & 32.6 & 86.9   & 81.0  & 83.9  & 74.6  &       &       &       &     &        &        &        &     \\
OpenIE 6                & ?                         & -    & -    & 52.7 & 33.7 &        &       &       &       & ?     & ?     & ?     & ?   & ?      & ?      & ?      & ?   \\
BERT\_base              & 109M                      & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 61.57 & 18.79 & 28.79 & ?   & 32.29? & 13.78? & 19.32? & ?   \\
BERT\_large             & 335M                      & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 61.69 & 18.99 & 29.05 & ?   & 29.08  & 18.61  & 22.70  & ?   \\
GPT-2                   & 117M                      & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 61.62 & 18.17 & 28.07 & ?   & ?      & ?      & ?      & ?   \\
GPT-2\_medium           & 345M                      & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 62.10 & 18.65 & 28.69 & ?   & ?      & ?      & ?      & ?   \\
GPT-2\_large            & 774M                      & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 62.38 & 19.00 & 29.12 & ?   & ?      & ?      & ?      & ?   \\
GPT-2\_xl               & 1558M                     & ?    & ?    & ?    & ?    & ?      & ?     & ?     & ?     & 62.69 & 19.47 & 29.72 & ?   & ?      & ?      & ?      & ?  \\
\end{tabular}%
}
\caption{}
\label{tab:my-table}
\end{table}
}

==> tabs/resulttac.tex <==
\begin{table}[t]
\centering
\resizebox{0.95\linewidth}{!}
  {
  \begin{tabular} {l | l | l | l | l}
    \toprule
    {\bf Method} & {\bf \#Params} & {\bf P\%} & {\bf R\%} & {\bf F1\%} \\
    \hline 
    % \hline
OpenIE 5.1 \footnoteref{ft:openie51}                            & - & 56.98                             & 14.54                              & 23.16                                                \\
Stanford OpenIE \citep{angeli2015leveraging}                             & - & 61.55                             & 17.35                              & 27.07                                                \\ 
RnnOIE \citep{stanovsky2018supervised}                             & - & ?                             & ?                              & ?    \\ 
OpenIE 6 \citep{kolluru2020openie6}                             & - & ?                             & ?                              & ?    \\ 
 \hdashline
BERT$_{\rm BASE}$                                      & 109M & 61.57                             & 18.79                              &  28.79                                               \\ 
BERT$_{\rm LARGE}$                        & 335M & 61.69                   & 18.99                     & 29.05                  \\ 
GPT-2                                    &  117M &   61.62                        & 18.17                             & 28.07                                              \\ 
GPT-2$_{\rm MEDIUM}$                                    & 345M & 62.10                             & 18.65                             &   28.69                                             \\
GPT-2$_{\rm LARGE}$                                    & \secbest 774M & 62.38                            & 19.00                             &  \secbest 29.12                                              \\
GPT-2$_{\rm XL}$                                    & \best 1558M & 62.69                            & 19.47                             &   \best 29.72 \electricblue{\tiny (+2.65)}                                              \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-0.1in}
\caption{{\small Compare the quality of relational knowledge on out-of-domain TAC KBP.}\xiao{add}}
\label{tab:resulttac}
\vspace{-0.1in}
\end{table}



\comm{
\begin{table}[t]
\centering
\resizebox{1.0\linewidth}{!}
  {
  \begin{tabular} {l | l | l | l | l}
    \toprule
    {\bf Method} & {\bf \#Params} & {\bf P\%} & {\bf R\%} & {\bf F1\%} \\
    \hline 
    % \hline
OpenIE 5.1 \footnoteref{ft:openie51}                            & - & 56.98                             & 14.54                              & 23.16                                                \\
Stanford OpenIE \citep{angeli2015leveraging}                             & - & 61.55                             & 17.35                              & 27.07                                                \\ 
% RnnOIE \citep{stanovsky2018supervised}                             & - & ?                             & ?                              & ?    \\ 
OpenIE 6 \citep{kolluru2020openie6}                             & - & ?                             & ?                              & ?    \\ 
 \hdashline
BERT$_{\rm BASE}$     (\electricblue{\small ours})                                  & 109M & 61.57                             & 18.79                              &  28.79                                               \\ 
BERT$_{\rm LARGE}$ (\electricblue{\small ours})                        & 335M & 61.69                   & 18.99                     & 29.05                  \\ 
GPT-2 (\electricblue{\small ours})                                    &  117M &   61.62                        & 18.17                             & 28.07                                              \\ 
GPT-2$_{\rm MEDIUM}$ (\electricblue{\small ours})                                    & 345M & 62.10                             & 18.65                             &   28.69                                             \\
GPT-2$_{\rm LARGE}$ (\electricblue{\small ours})                                    & \secbest 774M & 62.38                            & 19.00                             &  \secbest 29.12                                              \\
GPT-2$_{\rm XL}$ (\electricblue{\small ours})                                    & \best 1558M & 62.69                            & 19.47                             &   \best 29.72 (+2.65)                                              \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-0.1in}
\caption{{\small Compare the quality of mapped facts on TAC KBP. \#Params refers to the number of parameters of the pre-trained LM. P and R denote precision and recall.}\xiao{add}}
\label{tab:resulttac}
\vspace{-0.1in}
\end{table}
}

==> tabs/resultwiki.tex <==
\begin{table}[t]
\centering
\resizebox{0.95\linewidth}{!}
  {
  \begin{tabular} {l | l | l | l | l}
    \toprule
    {\bf Method} & {\bf \#Params} & {\bf P\%} & {\bf R\%} & {\bf F1\%} \\
    \hline 
    % \hline
    % \middlerule
        OpenIE 5.1 \footnoteref{ft:openie51}                            & - & 26.26?                             & 14.38?                              & 18.58?                                                \\
    Stanford OpenIE \citep{angeli2015leveraging}                           & - & 23.32                             & 13.09                              & 16.77 
    \\
    RnnOIE \citep{stanovsky2018supervised}                             & - & 28.51                                  & 14.65                             & 19.36  \\ 
    OpenIE 6 \citep{kolluru2020openie6}                             & - & ?                             & ?                              & ?    \\ 
    \hdashline
        BERT$_{\rm BASE}$                    & \secbest 109M  & 32.29?                   & 13.78?                    & \secbest 19.32?                 \\
    BERT$_{\rm LARGE}$                    & \best 335M  & 29.08                    & 18.61                    & \best 22.70 \electricblue{\tiny (+4.12)}                  \\
    % \method-GPT-2$_{\rm XL}$                     & \best 1558M  & 31.32                    & 17.42                    & \best 22.39 (+5.62)               \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-0.1in}
\caption{{\small Compare the quality of relational knowledge on in-domain Wikidata. \#Params refers to the number of parameters of the pre-trained LM. P and R denote precision and recall.}\xiao{add}}
\label{tab:resultwiki}
\vspace{-0.15in}
\end{table}

\comm{
\begin{table}[t]
\centering
\resizebox{1.0\linewidth}{!}
  {
  \begin{tabular} {l | l | l | l | l}
    \toprule
    {\bf Method} & {\bf \#Params} & {\bf P\%} & {\bf R\%} & {\bf F1\%} \\
    \hline 
    % \hline
    % \middlerule
    OpenIE 5.1 \footnoteref{ft:openie51}                            & - & ?                             & ?                              & ?                                                \\
    Stanford OpenIE \citep{angeli2015leveraging}                           & - & 23.32                             & 13.09                              & 16.77 
    \\
    % RnnOIE \citep{stanovsky2018supervised}                             & - & 28.51                                  & 14.65                             & 19.36  \\ 
    OpenIE 6 \citep{kolluru2020openie6}                             & - & ?                             & ?                              & ?    \\ 
    \hdashline
        BERT$_{\rm BASE}$ (\electricblue{\small ours})                    & \secbest 109M  & ?                    & ?                    & ?                 \\
    BERT$_{\rm LARGE}$ (\electricblue{\small ours})                    & \best 335M  & \best 29.52                    & \best 16.56                    & \best 21.22 \electricblue{\tiny (+?)}                  \\
    % \method-GPT-2$_{\rm XL}$ (\electricblue{\small ours})                     & \best 1558M  & 31.32                    & 17.42                    & \best 22.39 (+5.62)               \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-0.1in}
\caption{{\small Compare the quality of mapped facts on Wikidata.}\xiao{add}}
\label{tab:resultwiki}
\vspace{-0.15in}
\end{table}
}
